Stein Variational Gradient Descent as Moment Matching

Stein variational gradient descent (SVGD) is a non-parametric inference algorithm that evolves a set of particles to fit a given distribution of interest. We analyze the non-asymptotic properties of SVGD, showing that there exists a set of functions, which we call the Stein matching set, whose expectations are exactly estimated by any set of particles that satisfies the fixed point equation of SVGD. This set is the image of Stein operator applied on the feature maps of the positive definite kernel used in SVGD. Our results provide a theoretical framework for analyzing the properties of SVGD with different kernels, shedding insight into optimal kernel choice. In particular, we show that SVGD with linear kernels yields exact estimation of means and variances on Gaussian distributions, while random Fourier features enable probabilistic bounds for distributional approximation. Our results offer a refreshing view of the classical inference problem as fitting Stein's identity or solving the Stein equation, which may motivate more efficient algorithms.

==> icml2017/nongaussian.tex <==
\section{Linear Kernel for Non-Gaussian Distributions}
We showed that linear kernel yields exact estimation of mean and covariance when the target distribution $p$ is Gaussian. 
Here we should that when applying linear kernel to non-Gaussian distributions, the error on mean and covariance depends on 
the score function difference $\nabla_x\log p(x) = \nabla_x\log p^*(x)$, where $p^*$ is the best possible Gaussian distribution that approximates $p$. 

\begin{thm}




\end{thm}

First, assume $p^+(x)$ is normal distribution $\normal(\mu, \Sigma)$. Denote by $\steinpx^+$ its Stein operator, we have \begin{align*} 
\E_{\hat \mu_{X^*}}[\steinpx^+ \phi] 
-  \E_{p}[\steinpx^+ \phi]
& = \E_{\hat \mu_{X^*}}[\steinpx^+ \phi - \steinpx \phi ] 
-  \E_{p}[\steinpx^+ \phi - \steinpx \phi] \\
& = \E_{\hat \mu_{X^*} [ \delta_{p,p^+}(\vx) \phi(x) ]
- \E_{p} [ \delta_{p,p^+}(\vx) \phi(x) ].  
\end{align*} 
where $\delta_{p,p^+}(\vx) = \nabla_\vx\log p^+(\vx) - \nabla_\vx \log p(\vx)$. 
Taking $\phi(\vx) = \va^\top \vx + b$, we get
\begin{align*} 
\E_{\hat \mu_{X^*} - p}[\Sigma^{-1}(\vx-\vv\mu)(\vv a^\top \vx + b)] 
= \E_{\hat \mu_{X^*}-p} [ \delta_{p,p^+}(\vx) \phi(\vx) ]
\end{align*} 
Or 
\begin{align*} 
\E_{\hat \mu_{X^*}- p}[(\vx-\vv\mu)(\vv a^\top \vx + b)] 
= \E_{\hat \mu_{X^*}-p} [ \Sigma \delta_{p,p^+}(\vv a^\top\vx + b) \phi(\vx) ]
\end{align*} 
Taking $\vv a = 0$ and $b = 1$, we have 
\begin{align*} 
\E_{\hat \mu_{X^*} - p}[\vx] 
= \E_{\hat \mu_{X^*} - p} [ \Sigma \delta_{p,p^+}(\vx) ]
\end{align*} 
Therefore, 
\begin{align*} 
\norm{\E_{\hat \mu_{X^*} - p}[\vx] }_2^2
\leq 
\inf_{\mu,\Sigma}
\E_{\hat \mu_{X^*}} [\delta_{p,p^+}(\vx)^\top \Sigma^2 \delta_{p,p^+}(\vx)  ]  
+ \E_{p} [\delta_{p,p^+}(\vx)^\top \Sigma^2 \delta_{p,p^+}(\vx)  ]. 
\end{align*} 

For bounding the variance, take $\phi(\vx) = (\vx - \mu)^\top$. We have 
\begin{align*} 
%\norm{
\E_{\hat \mu_{X^*} - p}[ (x-\mu)(x-\mu)^\top]  
%}_2^2
\leq 
\inf_{\mu,\Sigma}
\E_{\hat \mu_{X^*}-p} [\Sigma \delta_{p,p^+}(\vx) (x - \mu)^\top
]
%\delta_{p,p^+}(\vx)^\top \Sigma^2 \delta_{p,p^+}(\vx)  ]  
%+ \E_{p} [\delta_{p,p^+}(\vx)^\top \Sigma^2 \delta_{p,p^+}(\vx)  ]. 
\end{align*} 

==> icml2017/tex/background.tex <==
\section{Background}
We introduce the basic background of
the Stein variational method, 
a framework of approximate inference that integrates ideas from Stein's method, 
kernel methods, and variational inference. 
The readers are referred to \citet{liu2016kernelized, liu2016stein, liu2017stein} and references therein for more details.
%\emph{Notation}
%
For notation, all vectors are assumed to be column vectors.
The differential operator $\nabla_{\vx}$ is viewed as a column vector of the same size as $\vx\in \RR^d$. For example,
$\nabla_\vx \phi$ is a $\RR^d$-valued function when $\phi$ is a scalar-valued function, and 
$\nabla_\vx^\top \ff(\vx) = \sum_{i=1}^d \partial_{x_i} \ff(\vx)$ is a scalar-valued function when $\ff$ is $\RR^d$-valued. 


\paragraph{Stein's Identity}
Stein's identity forms the foundation of our framework.  
Given a positive differentiable density $p(\vx)$ on $\mathcal X \subseteq \R^d$, one form of Stein's identity is 
$$ 
%\E_{x\sim p} [\langle \nabla_\vx \log p(\vx),~ \ff(\vx)\rangle  + \langle \nabla_\vx, ~ \ff(\vx)\rangle] =0, 
\E_p [\nabla_{\vx} \log p(\vx)^\top \ff(\vx) + \nabla_{\vx}^\top  \ff(\vx)] = 0, ~~~~~~ \forall \ff, 
$$ 
which holds for any differentiable, $\R^d$-valued function $\ff$ that satisfies a proper zero-boundary condition.  
Stein's identity can be proved by a simple exercise of integration by parts. 
\iffalse
taking the case  when $\X = \R$ as an example,  %we have 
\begin{align*}
& \E_{p} [\nabla_{\vx} \log p(\vx) \ff(\vx) + \nabla_{\vx} \ff(\vx)]  
%= \int \nabla_\vx p(\vx) \ff(\vx) + p(\vx) \nabla_\vx \ff(\vx) dx
 = \int \nabla_{x} (p(\vx) \ff(\vx)) d x  
 = p(\vx)\ff(\vx)\big |_{-\infty}^{+\infty} = 0. 
%p(+\infty) \ff(+\infty)  - p(-\infty) \ff(-\infty) = 0. 
\end{align*}
\fi
We may write Stein's identity in a more compact way by 
defining a Stein operator $\steinpx$:  
%For convenience, we define the \emph{Stein operator} $\steinpx$ formally as 
\begin{align*} 
\E_p [\steinpx^\top \ff(\vx)] = 0, && 
\text{where} &&\steinpx^\top \ff(\vx) =  \nabla_\vx \log p(\vx)^\top\ff(\vx)   + \nabla_\vx^\top \ff(\vx), 
%\steinpx \ff(\vx) = \langle \xnabla_\vx \log p(\vx),~ \ff(\vx)\rangle  + \langle \nabla_\vx, ~ \ff(\vx)\rangle. 
\end{align*}
%We may formally consider  $\steinpx  =  \nabla_\vx \log p + \nabla_\vx,$ 
%Formally, we ma
where $\steinpx$ is formally viewed 
as a $d$-dimensinoal column vector like $\nabla_\vx$, 
and hence $\steinpx^\top \ff$ is the inner product of $\steinpx$ and $\ff$, yielding a scalar-valued function. 
%This is a linear operator that acts on a scalar-valued function $\ff$ 
%and return a vector valued function. 
%Then, Stein's identity above becom%es  

The power of Stein's identity is that, for a given distribution $p$, it defines an \emph{infinite} number of functions of form $\steinpx^\top \ff$ that has zero expectation under $p$, 
all of which only depend on $p$ through the Stein operator $\steinpx$, or 
the score function $\nabla_\vx \log p(\vx) = \frac{\nabla p(\vx)}{p(\vx)},$ which is independent of the normalization constant in $p$ that is often difficult to calculate. 

\paragraph{Stein Discrepancy on RKHS}
Stein's identity can be leveraged to characterize the discrepancy between different distributions.  
The idea is that, for two different distributions $p\neq q$, 
there shall exist a function $\ff$ such that $\E_{q} [ {\steinpx^\top \ff}] \neq 0.$ 
Consider functions $\ff$ in a $\R^d$-valued reproducing kernel Hilbert space (RKHS) of form 
$\H = \H_0\times \cdots \H_0$ where $\H_0$ is a $\R$-valued RKHS with positive definite kernel $k(\vx, \vx')$. We may define a \emph{kernelized Stein discrepancy} (KSD) \citep{liu2016kernelized,chwialkowski2016kernel, oates2014control}:  
\begin{align}\label{ksdopt}
\S_k(q~||~ p) =\max_{\ff \in \H} \big \{  \E_{q} [\steinpx^\top \ff(\vx)] ~~\colon ||\ff ||_{\H} \leq 1 \big \},
\end{align}
%where $\H$ is a $\R^d$-valued function space equipped with a norm $|| \cdot||_\H$. 
%In particular, we take $\H$ to be a $\R^d$-valued reproducing kernel Hilbert space (RKHS) of form $\H = \H_0\times \cdots \H_0$ where $\H_0$ is a $\R$-valued RKHS with positive definite kernel $k(\vx, \vx')$. 
%with positive definition kernel $k(\vx,\vx')$\footnote{Here we assume $\H = \H_0\times \cdots \H_0$, where $\H_0$ is a real-valued RKHS with kernel $k(\vx, \vx')$.}
%In this case, the optimal $\ff$ in \eqref{ksdopt} has a simple closed form solution:
The optimal $\ff$ in  \eqref{ksdopt} can be solved in closed form: 
\begin{align}\label{ffstar}
\ff^*_{q,p}(\cdot) \propto \E_{\vx\sim q} [\steinpx k(\vx,\cdot)],
\end{align}
which yields a simple kernel-based representation of KSD:  %
\begin{align}\label{ksdkernel}
%\begin{split}
%\S^2(q~||~p) =  \E_{x,\vx'\sim q} [\steinpx^\top (\steinpxp k(\vx,\vx'))],
  \S^2_k(q~||~p) =  \E_{\vx,\vx'\sim q}  [\kappa_p(\vx,\vx') ], &
& \text{with}~~~~~~ \kappa_p(\vx,\vx') = \steinpx^\top(\steinpxp k(\vx,\vx')), 
%\end{split}
\end{align}
where $\vx$ and $\vx'$ are i.i.d. draws from $q$, 
and $\kappa_p(\vx,\vx')$ 
is a new ``Steinalized'' positive definite kernel obtained by applying the Stein operator twice, first w.r.t. variable $\vx$ and then $\vx'$. 
It turns out that the RKHS related to kernel $\kappa_p(\vx,\vx')$ 
is exactly the space of functions obtained by applying Stein operator on functions in $\H$, that is, 
$$
\H_p = \{  \steinpx^\top \ff  \colon \forall \ff \in \H  \}. 
$$
%Because $\steinpx$ is a linear operator, one can show that $\H_p$ is also a RKHS \citep{berlinet2011reproducing},  whose kernel is $\kappa_p(\vx,\vx')$ defined in \eqref{ksdkernel}. 
%$$
%\kappa_p(\vx,\vx') = \steinpx^\top(\steinpxp k(\vx,\vx')), 
%$$
%where $\steinp_{x} \otimes k(\vx,\cdot) = \nabla_\vx\logp(\vx)k(\vx,\cdot) +\nabla_\vxk(\vx,\cdot).$
%Here we apply Stein operator twice, first w.r.t. variable $x$ and then $x'$. 
By Stein's identity, all the functions in $\H_p$ have zero expectation under $p$. 
We can also define $\H_p^+$ 
to be the space of functions in $\H_p$ adding arbitrary constants, that is, $\H_p^+ := \{ f(\vx) + c \colon f \in  \H_p, ~~ c\in \R \}$, which can also be viewed as a RKHS, with kernel $\kappa_p(\vx,\vx') + 1$.  
%
Stein discrepancy can be viewed as a maximum mean discrepancy (MMD) on the Steinalized RKHS $\H_p^+$ (or equivalently $\H_p$): 
\begin{align}\label{shp}
\S_k(q~||~p) = \max_{f \in \H_p^+} \big\{   \E_q f - \E_p  f   \colon ~~~~~  || f||_{\H_p^+} \leq 1  \big\}. 
\end{align}
Different from typical MMD, 
here the RKHS space depends on distribution $p$.  
%
In order to make Stein discrepancy 
discriminative, in that $\S_k(q~||~p)=0$ implies $q=p$, 
we need to take kernels $k(\vx,\vx')$ so that $\H_p^+$ is sufficiently large. It has been shown that this can be achieved if $k(\vx,\vx')$ is strictly positive definite or universal, 
%or $\H$ is dense in the space of continuous functions,
in a proper technical sense  \citep{liu2016kernelized, chwialkowski2016kernel, gorham2017measuring, oates2014control}. 

%Intuitively speaking, one may consider strictly positive definite kernels as spanned by infinite number of linearly independent features. Consider the random feature representation, 
%It is consider to% 
%Consider the random feature representation 
It is useful to consider the kernels in a random feature representation \citep{rahimi2007random}, 
\begin{align}\label{kphi}
    k(\vx,\vx') = \E_{\vw\sim p_\vw}[\phi(\vx,\vw)\phi(\vx', \vw)], 
\end{align}
where $\phi(\vx,\vw)$ is a set of features indexed by a random parameter $\vw$ drawn from a distribution $p_\vw$. 
For example, the Gaussian RBF kernel $k(\vx,\vx') = \exp(-\frac{1}{2h^2}{||\vx-\vx'||^2_2})$ admits 
%Borcher's theorem showed that any stationary continuous kernel $k(\vx,\vx') = k(\vx - \vx')$ 
%can be represented using random Fourier features 
\begin{align}\label{cos}
\ff(\vx, \vw) = \sqrt{2} \cos(\frac{1}{h}\vw_1^\top \vx + w_0 ),
\end{align}
%under some distribution $p_w$. 
%For example, 
where $w_0\sim \mathrm{Unif}([0,2\pi])$ and $\vw_1 \sim \normal(0, I)$. 
%With \eqref{shp}, 
With the random feature representation, KSD can be rewritten into 
%But non-stationary kernels also have random feature expansion \citep{}. 
%With the random feature expansion \eqref{randk}, the kernel Stein discrepancy in \eqref{ksdkernel}  can be rewritten into 
\begin{align}
\label{ksdw}
\D_k^2(q~||~p) = 
% \E_{\vw} \sim p_{\vw} \bigg [\left {||} \E_{\vx \sim q} [\steinpx \ff(\vx, \vw)] \right{||}^2 \bigg ], \\
\E_{\vw \sim p_{\vw}} \bigg [|| \E_{\vx \sim q} [\steinpx \phi(\vx, \vw)] ||^2 \bigg ], 
\end{align}
which can be viewed as the mean square error of Stein's identity 
$\E_{\vx\sim q} [\steinpx \ff(\vx, \vw)] = 0$ over the random features. 
$\D_k^2(q~||~p) = 0$ shall imply $q = p$ if the feature set $\mathcal G = \{\ff(\vx, \vw)\colon \forall \vw\}$ is rich enough. 
Note that the RKHS $\H$ and feature set $\mathcal G$ are different; Stein discrepancy is an \emph{expected} loss function on $\mathcal G$ as shown in \eqref{ksdw},  
but a \emph{worst-case} loss on $\H$ as shown in \eqref{ksdopt}.  

%Then support of $p_w$ must be infinite for strictly positive definite kernels. In this work, however, we observe that it is sometimes beneficial to use \emph{degenerate} kernels formed by finite number of features, and the number of features is smaller than the particle size in use.

\paragraph{Stein Variational Gradient Descent (SVGD)}
SVGD is a deterministic sampling algorithm motivated by Stein discrepancy. It is based on the following basic observation: 
given a distribution $q$, assume $q_{[\ff]}$ is the distribution of $\vx' =\vx+ \epsilon \ff(\vx)$ obtained by updating $\vx$ with a velocity field $\ff$, where $\epsilon$ is a small step size, then we have 
%when $\vx\sim q$ and $\ff$ belongs to a RKHS $\H$, then 
$$
\KL(q_{[\ff]}~||~p) 
= \KL(q ~||~p)  - \epsilon \E_{q}[\steinpx^\top \ff] + O(\epsilon^2), 
%\frac{d\KL(q_{[\ff]}~||~p)}{d\ff} \big |_{\ff=0} = - \E_{q}[\steinpx^\top \ff], 
%\frac{d\KL(q_{[\ff]}~||~p)}{d\ff} \big |_{\ff=0} = - \E_{q}[\steinpx^\top \ff], 
$$
%where $\epsilon$ is a small step size.
which shows that the decrease of KL divergence 
 is dominated by $\epsilon\E_{q}[\steinpx^\top \ff]$. 
 In order to choose $\ff$ to make $q_{[\ff]}$ move towards 
 $p$ as fast as possible, we should choose $\ff$ to maximize $\E_{q}[\steinpx^\top \ff]$, whose solution is exactly $\ff^*_{q,p}(\cdot) \propto \E_{\vx\sim q} [\steinpx k(\vx,\cdot)]$ as shown in \eqref{ffstar}. 
 This suggests that $\ff^*_{q,p}$ happens to be the best velocity field that pushes the probability mass of $q$ towards $p$ as fast as possible.  

Motivated by this, SVGD approximates $q$ with the empirical distribution of a set of particles $\{\vx_i\}_{i=1}^n$, and iteratively updates the particles by 
%
\begin{align}\label{equ:update0}
\vx_i  \gets  \vx_i + \frac{\epsilon}{n} \sum_{j=1}^n 
[\steinp_{\vx_j} k(\vx_j,\vx_i)]. 
%[ \nabla_\vx \log p(\v\vx_i) k(\v\vx_i,\v\vx_j) + \nabla_{\vx_i} k(\v\vx_i,\v\vx_j)]. 
\end{align}
\citet{liu2017stein} studied the asymptotic properties of the dynamic system underlying SVGD, showing that the evolution of the limit density of the particles when $n\to\infty$ can be captured by a nonlinear Fokker-Planck equation, and established its weak convergence to the target distribution $p$. 


%The main weakness of 
However, the analysis in \citet{liu2017stein} and  \citet{lu2018scaling} do not cover the case when  the  sample size $n$ is finite, which is more relevant to the practical performance. We address this problem by directly analyzing the properties of the fixed point equation of SVGD, yielding results that work for finite sample size $n$, also independent of the update rule used to arrive the fixed points.  

==> icml2017/tex/draft.tex <==


\section{SVGD as Moment Matching}
This section presents our main results on the moment matching properties of SVGD and the related Stein matching sets. %  
%whose expectations are exactly estimated by SVGD.
We start with Section~\ref{sec:fixedsvgd} 
which introduces the basic idea and  
 characterizes the Stein matching set of SVGD with general positive definite kernels.   
We then analyze in Section~\ref{sec:featuresvgd} the special case when the rank of the kernel is less than the particle size, in which case 
the Stein matching set is independent of the fixed points themselves. 
Section~\ref{sec:gaussian} shows that 
SVGD with linear features exactly estimates the first two second-order moments of Gaussian distributions.
Section~\ref{sec:random} establishes 
%finite-sample concentration 
a probabilistic bound when random features are used.  

\subsection{Fixed Point of SVGD}\label{sec:fixedsvgd} 
%ignoring the dynamical perspective. 
%To be specific, assume $\{\vx_i^*\}$ is the fixed point of 
%\eqref{equ:update0}, it should satisfy   
%$$
% \frac{1}{n} \sum_{j=1}^n [ \steinp_{\vx_j} k(\v\vx_j,\v\vx_i)] = 0, ~~~~ \forall i = 1,\ldots, n. 
%$$
%\paragraph{Main Idea} 
Our basic idea is rather simple to illustrate. 
Assume $X^* = \{\vx_i^*\}_{i=1}^n$ is the fixed point of SVGD and $\hat\mu_{X^*}$ its related empirical measure, then according to \eqref{equ:update0}, 
the fixed point condition of SVGD ensures 
\begin{align}\label{equ:avgk}
%\avg{j}{1}{n }
\E_{\vx\sim \hat \mu_{X^*}} [ \steinp_{\vx} k(\vx,  \vx_i^*) ]  =  0, ~~~~~ ~~~~~ \forall i = 1, \ldots, n. 
\end{align}
On the other hand, by Stein's identity, we have 
$$
\E_{\vx\sim p} [\steinpx k(\vx, \vx_i^*)] =0,  ~~~~~ ~~~~~ \forall i = 1, \ldots, n. 
$$
This suggests that 
%all functions  of form $\steinpx k(\vx,\vx_i^*)$ have the same expectation under $\hat \mu$
$\hat\mu_{X^*}$ \emph{exactly} estimates the expectation of 
functions of form $f(\vx) = \steinpx k(\vx,\vx_i^*)$ under $p$, all of which are zero. 
%Because of 
By the linearity of expectation, the same holds for all the functions in the linear span of  $\steinpx k(\vx,\vx_i^*)$. 
%This can be 
%matches $p$ \emph{exactly} on the set of test functions that are linear span of $\steinpx k(\vx,\vx_i)$. 
%As a result, we have the following simple yet critical result, 
 \begin{lem}\label{lem:exact}
Assume $X^* = \{\vx_i^*\}_{i=1}^n$ satisfies the fixed point equation \eqref{equ:avgk} of SVGD. 
We have 
$$
\avg{i}{1}{n} f(\vx_i^* ) =  \E_p f, ~~~~~~~\forall f \in \mathcal F^*, 
$$
where the Stein matching set $\F^*$ is the linear span of $\{\steinpx k(\vx,\vx_i^*)\}_{i=1}^n \cup \{1\}$, that is, $\F^*$ consists of %is the set of functions of form 
\begin{align*}
 f(\vx) =  \sum_{i = 1}^n \vv a_i^\top  \steinpx k(\vx,\vx_i^*)~+~b, ~~~~~ \forall  \vv a_i\in \R^d,   ~ b \in \R. 
%\mathcal F_{X^*} = \{& x \mapsto  b ~+ ~ \sum_{i = 1}^n a_i^\top  \steinpx k(\vx,\vx_i)  \colon \\& ~~~~~~ b \in \R, ~~ a_i \in \R^d, ~\forall i = 1, \ldots, n       \}. 
\end{align*}
Equivalently, $f(\vx)  = \steinpx^\top \ff(\vx) + b$ and $\ff$ is in the linear span of $\{k(\vx, \vx_i^*)\}_{i=1}^n$, that is, $\ff(\vx) = \sum_{i=1}^n \vv a_i k(\vx, \vx_i^*). $
%where $a_i\in \R^d, ~ b \in \R,  ~i \in [n]
%\begin{align*}
%\mathcal F_{X^*} = 
%\{ x \mapsto  b ~+ ~ \sum_{i = 1}^n a_i^\top  \steinpx k(\vx,\vx_i)  \colon b \in \R, ~~ a_i \in \R^d, ~\forall i = 1, \ldots, n       \}.
%\end{align*}
%Then we have 
%that is, SVGD fixed points exactly estimate $\E_p f$,  $\forall f\in \mathcal F^*$. 
 \end{lem}
%The significance of Lemma~\ref{lem:exact} is that it identifies a space of functions whose expectation can be estimated exactly by any  fixed point of SVGD. %estimates exactly. 
%%This basic result holds for any fixed points of SVGD, 
%This is regardless of the iterative algorithm used to achieve the fixed points.  
%Therefore, it is applicable to cases when acceleration techniques are used to solve Equation~\ref{equ:avgk} in a faster fashion.   

Extending Lemma~\ref{lem:exact}, 
one can readily see that the SVGD fixed points can approximate the expectation of functions that are close to $\F^*$. Specifically, let $\F^*_{\epsilon}$ be the $\epsilon$ neighborhood of $\F^*$, that is, 
$\F_\epsilon^* = \{f \colon \inf_{f'\in \F} ||f -f'||_\infty \leq \epsilon  \},$ 
then it is easily shown that 
$$
\left | \avg{i}{1}{n} f(\vx_i^* ) -   \E_p f \right |  \leq 2 \epsilon, ~~~~~~~\forall f \in \mathcal F^*_\epsilon. 
$$
Therefore, the SVGD approximation can be viewed as \emph{prioritizing} the functions within, or close to, $\F^*$. This is different in nature from Monte Carlo, which approximates the expectation of \emph{all bounded variance functions} with the same $O(1/\sqrt{n})$ error rate. 
%
Instead, SVGD shares more similarity with the \emph{quadrature} and \emph{sigma point methods}, 
which also find points (particles) to match the expectation on certain class of functions, but mostly only on polynomial functions and for simple distributions such as uniform or Gaussian distributions. 
%
SVGD provides a more general approach that can match moments of richer classes of functions for more general complex multivariate distributions.  
As we show in Section~\ref{sec:gaussian}, when using polynomial kernels, SVGD reduces to matching  polynomials when applied to multivariate Gaussian distributions.  

In this view, the performance of SVGD is essentially decided by %depends on %, if is not fully determined by, 
the Stein matching set $\F^*$. We shall design the algorithm, by engineering the kernels or feature maps, to make 
$\F^*$ as large as possible in order to approximate the distribution well, or include the test functions
of actual interest, such as mean and variance.  %for query-specific inference. 

\subsection{Fixed Point of Feature-based SVGD}
\label{sec:featuresvgd}

One undesirable property of $\F^*$ in Lemma~\ref{lem:exact} is that it depends  
on the values of the fixed point particles $X^*$, whose properties are difficult to characterize \emph{a priori}. 
This makes it difficult to infer what kernel should be used to obtain a desirable $\F^*$. 
It turns out the dependency of $\F$ on $X^*$ can be essentially decoupled by using \emph{degenerated kernels} corresponding to a finite number of feature maps. 
Specifically, we consider kernels of form 
$$
k(\vx,\vx') = \sum_{\ell=1}^m \phi_\ell(\vx) \phi_\ell(\vx'), 
$$
%where $\phi_\ell\colon \X \to \R$ is a set of feature maps, 
where we assume the number $m$ of features is no larger than the particle size $n$. 
Then, the fixed point of SVGD reduces to 
\begin{align}\label{phi1}
 \E_{\vx\sim \hat\mu_{X^*}} [\sum_{\ell=1}^m \steinpx \phi_\ell(\vx) \phi_\ell(\vx_j^*) ]   = 0, ~~~~~\forall j\in [n]. 
\end{align}
Define $\Phi = [\phi_\ell(\vx_j^*)]_{\ell,j}$ which is a matrix of size $(m\times n)$ . If $rank(\Phi) \geq m$, then \eqref{phi1} reduces to 
\begin{align}
 \E_{\vx\sim \hat{\mu}_{X^*}} [\steinpx \phi_\ell(\vx)] = 0, 
 ~~~~~ \forall \ell=1,\ldots, m,
\end{align}
%This eliminates the dependency of the function that we take average over on the data
where the test function $f(\vx) := \stein_\vx \phi_\ell(\vx)$ no longer depends on the fixed point $X^*$.  %not depends
%This eliminates 
%Comparing with \eqre{phil}, the functions $\stein_$
\begin{thm}
\label{thm:phi}
Assume $X^*$ is a fixed point of SVGD with kernel $k(\vx,\vx') =\sum_{\ell=1}^m\phi_\ell(\vx)\phi_\ell(\vx')$. 
Define the $(m\times n)$ matrix $\Phi = [\phi_{\ell}(\vx_i^*)]_{\ell\in[m],i\in[n]}$.
If $\mathrm{rank}(\Phi) \geq m$, then 
$$
\frac{1}{n}\sum_{i=1}^n f(\vx_i^*) = \E_p f, ~~~~ \forall f\in \F^*, 
$$
where the Stein matching set $\F^*$ is the linear span of  $\{\steinpx \phi_\ell(\vx)\}_{\ell=1}^m \cup \{1\}$, that is, it is set of the functions of form 
\begin{align}\label{fellb}
\!\!\! f(\vx) =\sum_{\ell=1}^m \vv a_\ell^\top \steinpx \phi_\ell(\vx) ~+~  b, && 
\forall ~ \vv a_\ell \in \R^d, ~ b\in \R. 
\end{align}
%where $a_\ell \in \R^d$ and $b\in \R$. 
\end{thm}
%
Note that the rank condition implies that we must have $m \leq n$. The idea is that $n$ particles can at most match $n$ linearly independent features exactly. 
%using kernels with higher ranks does not seem to introduce 
Here, although the rank condition 
still depends on the fixed point $X^*=\{\vx^*_i\}_{i=1}^n$ and 
cannot be guaranteed \emph{a priori}, it can be numerically verified once we obtain the values of $X^*$. 
In our experiments, we find that the rank condition tends to always hold practically when $n=m$. In cases  when it does fail to satisfy, we can always rerun the algorithm with a larger $n$ until it is satisfied.  
Intuitively, it seems to require bad luck to have $\Phi$ low rank when there are more particles than features ($n\geq m$), although a theoretical guarantee is still missing. 
%and we can always increase $n$ if it is not satisfied. 
%practice, 
%especially when $n$ is significantly larger than $m$. %The key point is that once the rank condition is satisfied, the function set $\F_{X^*}$ on which SVGD fixed point exactly matches the target distribution is independent of the particular location of the solution $X^*$. 
%assume 
%We propose a variant of SVGD based on random feature that amends easier analysis, and good empirical performance. Our idea is the following: 
%we use degenerated kernel so that $$
%In order to avoid this, we can calculate the graphical models and 
%In general we would lik


\paragraph{Query-Specific Inference as Solving Stein Equation}
Assume we are interested in a \emph{query-specific} task of estimating $\E_p f$ for a specific test  function $f$. 
In this case, we should ideally select the features $\{\phi_\ell\}_\ell$ such that \eqref{fellb} holds to yield an exact estimation of $\E_p f$.  
By the linearity of the Stein operator, \eqref{fellb} is equivalent to 
\begin{align}\label{steineq}
\texttt{Stein Equation:} && 
f(\vx) = \steinpx^\top \ff(\vx) + b, 
\end{align}
where $\ff(\vx) = \sum_{\ell=1}^m \vv a_\ell \phi_\ell(\vx)$.  
Eq~\eqref{steineq} is known as \emph{Stein Equation} when solving $\ff$ and $b$ with a given $f$, which  effectively calculates the inverse of Stein operator. 

Stein equation plays a central role in Stein's method as a theoretical tool \citep{barbour2005introduction}. 
Here, we highlight its fundamental connection to the approximate inference problem: 
%inference problem can be essentially reduced to solving Stein equation: 
%it also provides a fundamental framework for inference:  
if we can exactly solve $\ff$ and $b$ for a given $f$,  
then the inference problem regarding $f$ is already solved (without running SVGD), since we can easily see that $\E_p f = b$ by taking expectation from both sides of \eqref{steineq}. 

Mathematically, this reduces the integration problem of estimating $\E_p f$ into solving a differential equation. 
It suggests that Stein equation is at least as hard as the inference problem itself, and we should not expect a tractable way to solve it in general cases. 
%
On the other hand, it suggested that efficient ways of approximate inference may be developed by approximate solutions of Stein equation. 
%See, for example, 
Similar idea has been investigated in  
\citet{oates2014control}, which 
developed a kernel approximation of Stein equation in the case based on a given set of points.
SVGD allows us to 
further extend this idea by optimizing the set of points (particles) on which approximation is defined. 
%Ideas have be
%\citep{oates2014control} can be viewed as 
%In fact, 
%On the other side, this suggest that we should not expect to solve Stein equation exactly in general cases since it is at least as hard as calculating $\E_p f$. This suggests that we can not expect to choose the features and kernels to match $\F^*$ with the functions of interest in general cases. 

\subsection{Linear Feature SVGD is Exact for Gaussian}
%\section{Exact Estimation for Gaussian Distribution}
\label{sec:gaussian}
%Since Stein equation is at least as hard as the inference problem itself, 
%we should not expect a tractable way to solve it, nor find a set of features to math $\F^*$ with a given set of test functions of interest.
%exactly in general cases, that is, it is generally difficult to steer  the choice of kernels and features to match $\F^*$ with the functions of interest. 
%
Although Stein equation is difficult to solve in general, 
it is significantly simplified when the distribution $p$ of interest is Gaussian. 
In the following, we show that when $p$ is a multivariate Gaussian distribution, 
we can use linear features, relating to a linear kernel $k(\vx,\vx') = \vx^\top \vx'+1$, to 
ensure that SVGD exactly estimates all the first and second order moments of $p$.  
%make $\F^*$ include all the first and second order moments. 
%This suggests that SVGD can \emph{exactly estimate} the mean and variance of a Gaussian when using linear kernels. 
This insight provides an important practical guidance on the optimal kernel choices for Gaussian-like distributions. 
%which appear widely in Bayesian inference thanks to 
\begin{thm}\label{thm:gaussian}
Assume $X^*$ is a fixed point of SVGD with polynomial kernel $k(\vx,\vx') = \vx^\top \vx' + 1$. 
Let $\F^*$ be the Stein matching set in Theorem \ref{thm:phi}. 
%in which $X^*$ yields exact estimation. 
%with exact estimation 
If $p$ is a multivariate normal distribution on $\R^d$, 
then $\F \subseteq \mathrm{Poly}(2)$, where $\mathrm{Poly}(2)$ 
is the set of all polynomials upto the second order, that is, 
$\mathrm{Poly}(2) = \{\vx^\top A \vx + \vv b^\top \vx +c \colon A\in \R^{d\times d}, ~ \vv b\in \R^d, ~ c\in \R \}$. 

Further, denote by $\Phi$ the $(d+1)\times n$ matrix defined by 
$$
\Phi =  \begin{bmatrix} 
\vx_1& \vx_2 & \cdots & \vx_n \\
1 & 1 & \cdots & 1 
\end{bmatrix}.
$$
If $\mathrm{rank}(\Phi) \geq d+1$, then $\F = \mathrm{Poly}(2)$. In this case, any fixed point of SVGD exactly estimates both the mean and the covariance matrix of the target distribution. 
\end{thm}
%\begin{proof}
%See Appendix~\ref{sec:gaussianproofproof}
%\end{proof}
%Because $X^*$ is a result of SVGD dynamics, we can not graunatee a priori if the rank condition $\mathrm{rank}(\bar X) \geq d+1$ is satistified. However, in practice, we can always check this condition after we get the fixed points, and increase the number of points if it is not satisfied. In practice, however, we find that this rank condition is always satisfied with $d+1$ points. It is an open question if all points that satisifes. 
%
%On the other hand, 
%In general, 
More generally, if the features are polynomials of order $j$, its related Stein matching set should be polynomials of order $j+1$ for Gaussian distributions. We do not investigate this further because 
it is less common to estimate higher order moments in multivariate settings.  %high dimensional cases.  

 Theorem~\ref{thm:gaussian} suggests that it is a good heuristic to include linear features in SVGD, 
because Gaussian-like distributions appear widely thanks to the central limit theorem and Bernstein–von Mises theorem, 
%and it is of common importance
and the main goal of inference is often to estimate the mean and variance. 
In contrast, the more commonly used Gaussian RBF kernel 
does not have similar exact recovery results for the mean and variance, even for Gaussian distributions. 
%has been shown to work %underestimate the variance when the dimension $d$ is high (see Figure~\ref{fig:gaussian_var}).  

A nice property of our result is that once we use fewer features than the particles and solve the fixed point exactly, 
the features do not ``interfere'' with each other. 
This allows us to ``program'' our algorithm by adding different types of features 
that serve different purposes in different cases. 
%and ensure that the result is good in different cases. 
%Therefore, in practice, we can simultaneously include different types of features that serve different purposes and ensure that the result is good in different cases. 
%including linear features that 
%and work well in different cases.

%This suggests that polynomial feature is particularly good for Gaussian distribution. In fact, it is certainly better than the more typical Gaussian RBF kernel, given that even the best bandwidth tend to underestimate the variance. 

%However, the weakness of polynomial kerenel is that it is not strictly positive definte, and its feature set is not large enough. Therefore, we need to add more feature. 
%Here is the idea (polynomial + random)... 


%We start with polynomial feature, and gradually add 
\iffalse
\begin{thm}
Assume $p$ and $\rho$    
\begin{align*}
\E_{\vx \sim p} [\mathcal Q_\vx \ff(\vx) ]  
& = \E_{\vx \sim p} [(\nabla_{\vx}\log p(\vx) - \nabla_{\vx}\log q(\vx))^\top \ff(\vx) ] \\
& \leq  \mathbb F(p~||~ q)^{1/2}  ||\ff(\vx)||_2 
\end{align*}
\end{thm}
\fi

==> icml2017/tex/experiments.tex <==
\section{Empirical Experiments} 

\begin{figure*}[ht]
\centering
%\textbf{Full range} \\
\begin{tabular}{ccccc}
\raisebox{1.5em}{\rotatebox{90}{\scriptsize Log10 MSE}}
\includegraphics[width=0.18\textwidth]{./figures/gaussian_identical_ex} &
\raisebox{1.5em}{\rotatebox{90}{\scriptsize Log10 MSE}}
\includegraphics[width=0.18\textwidth]{./figures/gaussian_identical_exsqr} &
\raisebox{1.5em}{\rotatebox{90}{\scriptsize Log10 MMD}}
\includegraphics[width=0.18\textwidth]{./figures/gaussian_identical_mmd} &
\raisebox{0.5em}{\rotatebox{90}{\scriptsize Estimated Variance}}
\includegraphics[width=0.18\textwidth]{./figures/gaussian_variance_nsamples_var_dim_100} &
\hspace{-28pt}
\raisebox{1.0em}{\includegraphics[width=0.12\textwidth]{./figures/random_feature_legend_s1}} \\
\scriptsize Number of samples & \scriptsize Number of samples &\scriptsize Number of samples & \scriptsize Number of samples &  \\
\small (a) $\E(x)$ &
\small  (b) $\E(x^2)$ &
\small  (c) MMD & 
% \small \multicolumn{2}{c}{(d) Estimated variance(true = $1$)}  \\
\small (d) Variance \\%Estimated variance(true = $1$)}  \\
\end{tabular}
\caption{
Results on standard Gaussian distribution ($d=100$). 
	(a)-(b) show the MSE when using the obtained particles to 
	estimate the mean and second order moments of each dimension, averaged across the dimensions. 
	(c) shows the maximum mean discrepancy between the particle distribution and true distribution. 
	(d) shows the average values of the estimated variance (the true variance is 1).
}
\label{fig:gaussian_eh}
\end{figure*}


\begin{figure*}[ht]
\centering
\begin{tabular}{ccccc}
{\scriptsize ~~Condition number = 10} & 
{\scriptsize ~~Condition number = 10}  &
{\scriptsize ~~Number of samples = 250} & 
{\scriptsize ~~Number of samples = 250} &  \\
\raisebox{1.5em}{\rotatebox{90}{\scriptsize Log10 MSE}}
\includegraphics[width=0.18\textwidth]{./figures/gaussian_cond_10_nsampels_var_dim_100_ex} &
\raisebox{1.5em}{\rotatebox{90}{\scriptsize Log10 MSE}}
\includegraphics[width=0.18\textwidth]{./figures/gaussian_cond_10_nsampels_var_dim_100_exsqr} &
\raisebox{1.5em}{\rotatebox{90}{\scriptsize Log10 MSE}}
\includegraphics[width=0.18\textwidth]{./figures/gaussian_cond_var_nsamples_250_ex} &
\raisebox{1.5em}{\rotatebox{90}{\scriptsize Log10 MSE}}
\includegraphics[width=0.18\textwidth]{./figures/gaussian_cond_var_nsamples_250_exsqr} &
% \raisebox{3.2em}{\rotatebox{90}{\small Log10 MMD}}
% \includegraphics[width=0.25\textwidth]{./figures/gaussian_cond_var_nsamples_250_mmd}  & 
\hspace{-28pt}
\raisebox{0.5em}{\includegraphics[width=0.12\textwidth]{./figures/random_feature_legend}} \\
\scriptsize Number of samples &\scriptsize Number of samples & \scriptsize Condition Number &\scriptsize Condition Number   \\
(a)~$\E(x)$ & (b)~$\E(x^2)$ & (c)~$\E(x)$ & (d)~$\E(x^2)$\\
\end{tabular}
\caption{(a)-(b) Results on random $100$ dimensional non-spherical Gaussian distributions whose covariance matrix has a conditional number of ${\lambda_{\max}}/{\lambda_{\min}} = 10$. 
(c)-(d) 
The performance on random non-spherical Gaussian distributions with different conditional numbers. 
%for SVGD(Linear+Random) and SVGD(linear), larger conditional numbers give worse performance because of numerical errors.  
%t%he performance deteorates as n
%shows the MSE vs. the condition number ,  we use a fixed particle size of $n=250$. (c)-(d) shows the MSE vs. the particle size $n$, 
%with fixed condition number ${\lambda_{\max}}/{\lambda_{\min}} = 10$. 
Results averaged on 20 random models.  
}
\label{fig:gaussian_cond_var}
\end{figure*}


Our results show that linear features 
allow us to obtain accurate estimates of the first and second moments for Gaussian-like distributions, 
while random features can obtain a good overall distributional approximation with high probability. 
To test these theoretical observations empirically, 
we design a ``linear+random'' kernel: 
\begin{align*}
%\label{linrnd}
%\!\!\!\!\!\!\!
k(\vx,\vx') &= 
\alpha ( 1 + {\vx}^\top {\vx}') 
 + \beta \!\!\sum_{\ell = d+2}^n\!\! \phi(\vx, \vw_\ell) \phi(\vx', \vw_\ell), 
\end{align*}
where we take $\alpha = {{1}/({d+1})} $ and $\beta = {1}/{(n-d-1)}$ in our experiments. 
In the case when there are fewer particles than dimension plus one ($n {\leq} d+1$), we have $k({\vx}, {\vx}') = 1+ {\vx}^\top {\vx}'$, which only include the linear features, and when $n> (d+1)$, additional random features are added, so that the total number of features matches the number of particles.
%The idea of using kernel of rank $n$, instead of universal kernels with infinite rank, is that with $n$ data points, at most $n$

%In our experiments, 
We take $\phi(\vx,\vw)$ to be the random cosine 
feature in \eqref{cos} to approximate the Gaussian RBF kernel. 
%
Note that in our method, the random parameters $\{\vw_\ell\}$ are drawn in the beginning and fixed across the iterations of the algorithm, but we adopt the bandwidth $h$ across the iterations using the median trick. 
%Therefore, technically speaking, $h$ would also depend on the fixed point $X^*$. %This does not break our theory because
%We use AdaGrad optimizer with momentum unless otherwise specified.
We compare exact Monte Carlo with SVGD with different kernels, 
including the standard Gaussian RBF kernel, the linear kernel $k({\vx}, {\vx}') = 1+ {\vx}^\top {\vx}'$, and the linear+random kernel defined above. 

\textbf{Gaussian Models}
We start with verifying our theory on 
a simple standard Gaussian distribution $p(\vx)=\normal(\vx, 0,I)$ with $d=100$ dimensions.
In Figure~\ref{fig:gaussian_eh}, we can see that all SVGD methods estimate the mean parameters  exceptionally well (Figure~\ref{fig:gaussian_eh}(a)). 
Variance estimation is more difficult for SVGD in general, 
but both the Linear+Random and Linear kernels perform well as the theory predicts: 
the errors drop quickly as $n$ approaches $d+1$ (the minimum particle size needed to recover mean and covariance matrices), and only the numerical error is left when $n>d+1$. 

To examine the variance estimation more closely, 
we show in Figure \ref{fig:gaussian_eh}(d) the value of the estimated variance (averaged across the dimensions) on the same 100-dimensional standard Gaussian distribution. 
%
We find that all the variants of SVGD tend to underestimate the variance when there is insufficient number of particles (in particular, when $n<d+1$), 
but the kernels that include linear features give (near) exact estimation once $n\geq d+1$. 

Figure~\ref{fig:gaussian_cond_var} shows a similar plot 
for 100-dimensional non-spherical Gaussian distributions when the conditional number of the covariance matrix varies. 
%conditional number $\lambda_{\max}/\lambda_{\min}$ of $\Sigma$ varies. 
In particular, we set $p(\vx) = \mathcal N(\vx;~\vv\mu, \Sigma)$ where $\vv \mu\sim \mathrm{Unif}([-3,3])$ and $\Sigma = I + \alpha \Lambda\Lambda^\top$, 
 with the elements of $\Lambda$ drawn from $\normal(0,1)$ and 
$\alpha$ adjusted to make the conditional number $\lambda_{\max}/\lambda_{\min}$  of $\Sigma$ equal  specific numbers. 
When the condition number equals $1$, we should have $\Sigma = I$.

Figure~\ref{fig:gaussian_cond_var}(a)-(b) show the estimation of the first and second order moments 
when the conditional number equals 10, in which SVGD(linear+random) and SVGD(linear) 
again show a near exact recovery after $n>d+1$. 
Figure~\ref{fig:gaussian_cond_var}(c)-(d) show that as the conditional number increases, 
the accuracy of all the methods decreases, but SVGD(linear+random) and SVGD(linear) still significantly outperform Monte Carlo estimation. 
%
The increased errors in SVGD(linear+random) and SVGD(linear) are caused by the increase of numerical
error because it is more difficult to satisfy the fixed point equation with high accuracy when the conditional number is large. 
%because our theory predicts exactly recovery for \emph{arbitrary} Gaussian distribution once the fixed point equation holds exactly. 


\newcommand{\tmpht}{0.15}
\begin{figure*}[ht]
\centering
\begin{tabular}{ccccc}
\raisebox{1.0em}{\rotatebox{90}{\scriptsize Relative MSE}}
\includegraphics[height=\tmpht\textwidth]{./figures/gmm_alpha_var_dim_10_nsamples_100_ex} &
\raisebox{1.0em}{\rotatebox{90}{\scriptsize Relative MSE}}
\includegraphics[height=\tmpht\textwidth]{./figures/gmm_alpha_var_dim_10_nsamples_100_exsqr} &
%\raisebox{1.0em}{\rotatebox{90}{\scriptsize Relative MSE}}
%\includegraphics[width=\tmpht\textwidth]{./figures/gmm_alpha_var_dim_10_nsamples_100_excos} &
\raisebox{1.0em}{\rotatebox{90}{\scriptsize Relative MMD}}
\includegraphics[height=\tmpht\textwidth]{./figures/gmm_alpha_var_dim_10_nsamples_100_mmd}  & 
\hspace{-5 pt}
\raisebox{3.8em}{\includegraphics[width=0.15\textwidth]{./figures/random_feature_legend}} \\
Gaussianity $\alpha$ & Gaussianity $\alpha$  &  Gaussianity $\alpha$ \\
$\E(x)$ & $\E(x^2)$ & MMD &  \\
\end{tabular}
\label{fig:gmm_alpha}
\caption{
Results on Gaussian mixture models $p(\vx)=\sum_{k=1}^{15}\normal(\alpha\vv\mu_{k},I)$, where $\vv\mu_k \sim \mathrm{Uniform}([0,1])$ and $\alpha$ controls the Gaussianity of $p$ (when $\alpha=0$, $p$ is standard Gaussian). All the results are the relative performance w.r.t. exact Monte Carlo sampling 
method with the sample size (we fix  for all the methods). 
%All results are 
We fix $n=100$ for all the methods and average the result over $20$ {random models}. 
}
\end{figure*}
\vspace{5pt}

\begin{figure*}[ht]
\centering
\begin{tabular}{ccccc}
\raisebox{1.5em}{\rotatebox{90}{\scriptsize Log10 MSE}}
\includegraphics[height=\tmpht\textwidth]{./figures/rbm_nsamples_var_dim_100_ex} &
\raisebox{1.5em}{\rotatebox{90}{\scriptsize Log10 MSE}}
\includegraphics[height=\tmpht\textwidth]{./figures/rbm_nsamples_var_dim_100_exsqr} &
%\raisebox{1.5em}{\rotatebox{90}{\scriptsize Log10 MSE}}
%\includegraphics[height=\tmpht\textwidth]{./figures/rbm_nsamples_var_dim_100_excos} &
\raisebox{1.5em}{\rotatebox{90}{\scriptsize Log10 MMD}}
\includegraphics[height=\tmpht\textwidth]{./figures/rbm_nsamples_var_dim_100_mmd}  & 
\hspace{-5pt}
\raisebox{3.8em}{\includegraphics[width=0.15\textwidth]{./figures/random_feature_legend}} \\
Number of samples & Number of samples   & Number of samples \\
$\E(x)$ & $\E(x^2)$  & MMD &  \\
\end{tabular}
\label{fig:gaussian_rbm}
\caption{
Results on randomly generated Gaussian-Bernoulli RBM, averaged on $20$ trials. 
%(a)-(c) The MSE for estimating 
%(c) for $\cos(wx+b)$, we random draw $w \sim \N(0,1)$ and $b\sim \mathrm{Uni}([2, 2\pi])$.
%
}
\end{figure*}

\paragraph{Gaussian Mixture Models}
We consider a Gaussian mixture model with density fucntion 
$p(\vx) = \frac{1}{15}\sum_{j=1}^{15} \normal(\vx; \alpha \vv\mu_{j}, ~ I),$ 
where $\vv\mu_{j}$ is randomly drawn from $\mathrm{Unifrom}([0, 1])$, 
and $\alpha$ can be viewed as controlling the Gaussianity of $p(\vx)$: 
when $\alpha$ equals zero, $p(\vx)$ reduces to the standard Gaussian distribution,
while when $\alpha$ is large, $p(\vx)$ would be highly multimodal with mixture components far away from each other.

\myempty{
To deal with multimodality, 
we leverage the idea of \emph{annealing} and
move the particles from a simple prior distribution to our target 
via a sequence of intermediate distributions.
Let $p_0$ be a prior distribution that is easy to 
approximate, we define a path of distributions that 
interpolate between prior $p_0$ and target $p$,
$$
p_\ell \propto p_0(x)^{1-\alpha_\ell}p(x)^{\alpha_\ell},
$$
where $0 = \alpha_0 < \cdots < \alpha_T = 1$
is a set of temperatures, and $T$
is the number of annealing steps.
Our algorithm starts from a set of particle
$\{x_i^0\}_{i=1}^n$ drawn from $p_0$, and then
moves the particles $\{x_i^\ell\}_{i=1}^n$
to approximate intermediate distribution $p_\ell$ sequentially by running
a small number of steps ($=20$) of SVGD updates.
We select $p_0 = \normal(0, 10^2)$ and use a annealing steps $T=1000$.
}

Figure~\ref{fig:gmm_alpha} shows the relative performance of SVGD with different kernels compared to exact Monte Carlo sampling. We find that SVGD methods generally outperform Monte Carlo unless $\alpha$ is very large. 
In Figure~\ref{fig:gmm_alpha}(b),
we can see that SVGD(Linear) outperforms SVGD(RBF) when
 $p$ is close to Gaussian (small $\alpha$), 
and performs worse than SVGD(RBF) when $p$ is highly non-Gaussian (large $\alpha$).  
SVGD(Linear+Random) combines the advantages of both and 
tends to match the best of SVGD(Linear) and SVGD(RBF) in all the range of $\alpha$. 

\paragraph{Gaussian-Bernoulli RBM} 
Gaussian-Bernoulli RBM is a
hidden variable model consisting of a continuous observable
variable $\vv x\in \R^d$ and a binary hidden variable $\vv h\in\{\pm 1\}^{d'}$ with probability
$$
% p(z, h) \propto \exp(\frac{1}{2} x^\top Bh + b^\top z + c^\top h - \frac{1}{2}||z||_2^2)
p(\vx, \vv h) \propto \sum_{\vv h\in \{\pm\}^{d'}} 
\exp( \vx^\top B\vv h + \vv b^\top \vv x + \vv c^\top \vv h - \frac{1}{2}||\vx||_2^2), 
$$
where we  randomly draw $\vv b$ and $\vv c$ from $\normal(0, I)$, 
and the elements of $B$ from $\mathrm{Uniform}(\{\pm 0.1\})$. 
We use $d=100$ observable variables and $d'=10$ hidden variables, 
so $p(\vv x)$ is effectively a Gaussian mixture with $2^{10}$ components.  
The results are shown in Figure~\ref{fig:gaussian_rbm}, where we find that 
SVGD(Linear+Random) again achieves the best performance in terms of all the evaluation metrics. 



% \begin{figure*}[ht]
% \centering
% %\textbf{Full range} \\
% \begin{tabular}{cccc}
% \raisebox{3.2em}{\rotatebox{90}{\small Log10 MSE}}
% \includegraphics[width=0.25\textwidth]{./figures/gaussian_identical_ex} &
% \includegraphics[width=0.25\textwidth]{./figures/gaussian_identical_exsqr} &
% \raisebox{3.2em}{\rotatebox{90}{\small Log10 MMD}}
% \includegraphics[width=0.25\textwidth]{./figures/gaussian_identical_mmd} &
% \raisebox{3em}{\includegraphics[width=0.15\textwidth]{./figures/gaussian_legend}} \\
% Number of samples & Number of samples & Number of samples &  \\
% $\E(x)$ & $\E(x^2)$ & MMD & \\
% \end{tabular}
% \label{fig:gaussian_eh}
% \caption{Identical Gaussian, dimension = 100, same settings as before.}
% \end{figure*}



% \section{Practical Algorithm and Experiments}
% Our results show that we should use both linear features 
% to obtain accurate estimation of the first and second moments for Gaussian-like distributions, 
% and also random features to obtain obtain a good distributional approximation overall. This motivates us use a ``Linear+Random'' kernel 
% $$
% k(\vx,\vx') = \red{\frac{1}{d+1}} 1 + \vx^\top \vx' + \frac{1}{n-d-1}\sum_{\ell = d+2}^n \phi(\vx, \vw_\ell) \phi(\vx, \vw_\ell), 
% $$
% where $\phi(x, w)$ is a typical random feature. In the case when $n \leq d+1$, we use $k(\vx, \vx') = 1+ \vx^\top \vx^'$ all the linear features. 

% In particular, we use random Fourier feature which corresponds to Gaussian RBF kernel $k(\vx,\vx') = \exp(-\frac{||\vx-\vx'||^2_2}{2h^2})$: 
% $$
% \phi(\vx,\vw) = \sqrt{2}\cos(\frac{1}{h}\vw_1^\top \vx + w_0),
% $$
% where $\vw = [w_0, \vw_1]$, and $w_0\sim \mathrm{Unif}([0,2\pi])$ and $\vw \sim \normal(0, I)$, and $h$ is the bandwidth parameter.  
% Note that in our method, the random parameters $\{\vw_\ell\}$ are drawn in the beginning and fixed across the iterations of the algorithm. 
% We adopt the bandwidth $h$ across the iterations using the median trick. Therefore, technically speaking $h$ would also depend on the fixed point $X^*$. 
% We use AdaGrad optimizer with momentum $0.9$ unless otherwise specified.


% Figure~\ref{fig:gaussian_eh} 
% compares the Linear+Random SVGD with exact Monte Carlo and SVGD with the typical RBF kernel on a 100 dimensional standard Gaussian distribution. 
% We can see that all SVGD estimates the mean parameter exceptionally well (Figure~\ref{fig:gaussian_eh}(a)). both the Linear+Random and Linear-only kernels \emph{exactly} estimate the second order moment once $n \geq d+1$ as predicted by our theorem, while the RBF kernel does worse on estimating the second moments  (Figure~\ref{fig:gaussian_eh}). 
% Figure~\ref{fig:gaussian_eh} shows the MMD between the SVGD fixed point and target distribution where we observe that MMD decays with a $O(1/\sqrt{n})$ rate once the random features kicks in when $n \geq d+1$. Figure~\ref{fig:gaussian_eh_none} shows a similar plot for 100 dimensional non-standard Gaussian $p(x) = \N(x;~\mu, \Sigma)$ 
% with random $\mu\sim \mathrm{Unif}([-3,3])$ and 
% condition number $\frac{|\lambda_\max|}{|\lambda_\min|}$ equals to $10$,
% where $\lambda_\max$ and $\lambda_\min$ are maximal and 
% minimal eigenvalues of $\Sigma$ respectively.
% % $\Sigma = 10 I + 0.1 \vv e^\top \vv e$ where $\vv e$ is the $\R^d$ column vector of all ones. 

% It is of particular interest to exam the estimation of the variance given by SVGD particles. Figure \ref{fig:gaussian_var} shows the estimated variance (averaged across the dimensions) over standard Gaussian distribution with different dimensions. We find that RBF SVGD  typically underestimate the true variance (which equals one) and requires increasingly more samples to obtain accurate variance estimation in higher dimensions, 
% while by adding the linear features, we again obtain the exact variance estimation once $n \geq d+1$. 
% % since it estimates the amount of 


% \begin{figure*}[ht]
% \centering
% \begin{tabular}{cccc}
% \raisebox{3.2em}{\rotatebox{90}{\small Variance}}
% \includegraphics[width=0.25\textwidth]{./figures/var_dim_10} &
% \includegraphics[width=0.25\textwidth]{./figures/var_dim_50} &
% \includegraphics[width=0.25\textwidth]{./figures/var_dim_100} &
% \raisebox{6em}{\includegraphics[width=0.15\textwidth]{./figures/var_legend}} \\
% (a) Dim = 10 & (b) Dim = 50 & (c) Dim = 100 & \\
% \end{tabular}
% \caption{The variance estimation of standard normal distributions with different dimensions. SVGD with the typical RBF kernel tends to underestimate the variance, while by using linear features, SVGD exactly estimates the variance when $d \geq d+1$.}
% \label{fig:gaussian_var}
% \end{figure*}



% \begin{figure*}[ht]
% \centering
% \begin{tabular}{cccc}
% \raisebox{3.2em}{\rotatebox{90}{\small Log10 MSE}}
% \includegraphics[width=0.25\textwidth]{./figures/gau_cond_10_nsamples_var_ex} &
% \includegraphics[width=0.25\textwidth]{./figures/gau_cond_10_nsamples_var_exsqr} &
% \raisebox{3.2em}{\rotatebox{90}{\small Log10 MMD}}
% \includegraphics[width=0.25\textwidth]{./figures/gau_cond_10_nsamples_var_mmd}  & 
% \raisebox{3em}{\includegraphics[width=0.15\textwidth]{./figures/gau_cond_10_nsamples_var_legend}} \\
% Number of samples & Number of samples & Number of samples   & \\
% $\E(x)$ & $\E(x^2)$ & MMD  & \\
% \end{tabular}
% \label{fig:gaussian_eh_none}
% \caption{Condition Number = 10; Gaussian distribution with 100 dimensions. }
% \end{figure*}


% \paragraph{Gaussian-Bernoulli RBM} 
% Gaussian-Bernoulli RBM is a
% hidden variable model consisting of a continuous observable
% variable $x\in \R^d$ and a binary hidden variable $h\in{\pm 1}^\ell$ with joint probability
% $$
% % p(z, h) \propto \exp(\frac{1}{2} x^\top Bh + b^\top z + c^\top h - \frac{1}{2}||z||_2^2)
% p(z, h) \propto \exp( x^\top Bh + b^\top z + c^\top h - \frac{1}{2}||z||_2^2)
% $$
% where the parameters include $\theta=\{B, b, c\}$.
% We take $\ell =10$ hidden variables and $d=100$ observable variables, and randomly draw $b$ and $c$ from $\N(0, 1)$, and $B$ is uniformly drawn from \{\pm 0.1\}. 
% % \begin{figure*}[ht]
% % \centering
% % \begin{tabular}{cccc}
% % \raisebox{3.2em}{\rotatebox{90}{\small Log10 MSE}}
% % \includegraphics[width=0.23\textwidth]{./figures/rbm_01_ex} &
% % \includegraphics[width=0.23\textwidth]{./figures/rbm_01_exsqr} &
% % \raisebox{3.2em}{\rotatebox{90}{\small Log10 MMD}}
% % \includegraphics[width=0.23\textwidth]{./figures/rbm_01_mmd}  & 
% % \raisebox{3em}{\includegraphics[width=0.15\textwidth]{./figures/rbm_legend}} \\
% % Number of samples & Number of samples & Number of samples  &  \\
% % $\E(x)$ & $\E(x^2)$ & MMD &  \\
% % \end{tabular}
% % \label{fig:rbm_01}
% % \caption{Results on Gaussian-Bernoulli RBM.}
% % \end{figure*}

% \begin{figure*}[ht]
% \centering
% \begin{tabular}{cccc}
% \raisebox{3.2em}{\rotatebox{90}{\small Log10 MSE}}
% \includegraphics[width=0.23\textwidth]{./figures/rbm_nsamples_var_dim_100_ex} &
% \includegraphics[width=0.23\textwidth]{./figures/rbm_nsamples_var_dim_100_exsqr} &
% \raisebox{3.2em}{\rotatebox{90}{\small Log10 MMD}}
% \includegraphics[width=0.23\textwidth]{./figures/rbm_nsamples_var_dim_100_mmd}  & 
% \raisebox{3em}{\includegraphics[width=0.15\textwidth]{./figures/rbm_nsamples_var_dim_100_legend}} \\
% Number of samples & Number of samples & Number of samples  &  \\
% $\E(x)$ & $\E(x^2)$ & MMD &  \\
% \end{tabular}
% \label{fig:rbm_01}
% \caption{Results on Gaussian-Bernoulli RBM.}
% \end{figure*}

% \paragraph{Gaussian Mixture Models}

% We consider a Guassian Mixture model with 15 components,
% $$
% p(x) = \frac{1}{15}\sum_{j=1}^{15} \N(x; \mu_{jk}, \sigma^2), ~~~k = 1, \cdots, 10
% $$
% where $\mu_{jk}$ is randomly drawn from $\mathrm{Unifrom}(0, \alpha)$.
% The variance $\sigma^2$ is set to $1$.
% The $\alpha$ is used to adjust the Gaussianity of $p(x)$. With $\alpha=0$,
% all components are overlaped with each other,  $p(x)$ is a standard Gaussian distribution. With larger $\alpha$, $p(x)$ could be  highly multi-model and components are far away from each other.


% Figure xx shows the MSE of different algorithms when estimating the
% posterior mean $\E_p[h(x)]$ with xxxx.
% The number of samples we used is $100$.

% \begin{figure*}[ht]
% \centering
% \begin{tabular}{cccc}
% \raisebox{3.2em}{\rotatebox{90}{\small Log10 MSE}}
% \includegraphics[width=0.23\textwidth]{./figures/gmm_alpha_var_max_5_dim_10_nsamples_100_ex} &
% \includegraphics[width=0.23\textwidth]{./figures/gmm_alpha_var_max_5_dim_10_nsamples_100_exsqr} &
% \raisebox{3.2em}{\rotatebox{90}{\small Log10 MMD}}
% \includegraphics[width=0.23\textwidth]{./figures/gmm_alpha_var_max_5_dim_10_nsamples_100_mmd}  & 
% \raisebox{3em}{\includegraphics[width=0.15\textwidth]{./figures/gmm_alpha_var_max_5_dim_10_nsamples_100_legend}} \\
% alpha & alpha & alpha  &  \\
% $\E(x)$ & $\E(x^2)$ & MMD &  \\
% \end{tabular}
% \label{fig:rbm_01}
% \caption{GMM, dim = 10, number of samples =100.}
% \end{figure*}

==> icml2017/tex/introduction.tex <==
\section{Introduction}
One of the core problems of modern statistics and machine learning is to approximate difficult-to-compute probability distributions.
Two fundamental ideas have been extensively studied and used in the literature: 
 variational inference (VI) and Markov chain Monte Carlo (MCMC) sampling \citep[e.g.,][]{koller2009probabilistic, wainwright2008graphical}. 
MCMC has the advantage of being non-parametric and asymptotically exact, 
but often suffers from difficulty in convergence, 
while VI frames the inference into a parametric optimization of the KL divergence and works much faster in practice, but loses the asymptotic consistency.  
An ongoing theme of research is to combine the advantages of these two methodologies. 

Stein variational gradient descent (SVGD) \citep{liu2016stein} is a synthesis of MCMC and VI that inherits the non-parametric nature of MCMC while maintaining the optimization perspective of VI. In brief, SVGD for distribution $p(x)$ updates a set of particles $\{\vx_i\}_{i=1}^n$ parallelly with 
%iteratively by $\vx_i  \gets \vx_i + \epsilon \ff(\vx_i)$, $\forall i =1,\ldots,n$, where $\ff(\cdot)$ is 
a velocity field $\ff(\cdot)$ that balances the gradient force and repulsive force, 
\begin{align*}
\vx_i  \gets \vx_i + \epsilon \ff(\vx_i), &&
%\vx_i  \gets \vx_i  + 
\ff(\cdot) = 
\frac{1}{n} \sum_{j=1}^n \nabla_{\vx_j} \log p(\vx_j) k(\vx_j, \cdot) +  \nabla_{\vx_j} k(\vx_j, \cdot), 
\end{align*}
where $\epsilon$ is a step size and $k(\vx,\vx')$ is a positive definite kernel defined by the user.
This update is derived as approximating a kernelized Wasserstein gradient flow of KL divergence \citep{liu2017stein} with connection to 
Stein's method \citep{stein1972} and  
optimal transport \citep{ollivier2014optimal}; 
see also \citet{tmpsuk}. 
%motivated by a connection between Stein's method \citep{stein1972} and KL divergence. 
%Based on a new observation that connects Stein's method \citep{stein1972} with KL divergence, SVGD is derived as a new type of functional gradient descent on the KL divergence in the  space of distributions, which is practically approximated non-parametrically  
%with a particle dynamical system that drives a set of particles to fit the distribution of interest. 
%by following the gradient direction while remaining a proper diversity via a repulsive force. 
%
SVGD has been applied to solve challenging inference problems in various domains; 
examples include Bayesian inference \citep{liu2016stein, feng2017learning}, uncertainty quantification \citep{zhu2018bayesian}, reinforcement learning \citep{liu2017stein, haarnoja2017reinforcement},  learning deep probabilistic models  \citep{wang2016learning, pu2017vae} 
and Bayesian meta learning \citep{feng2017learning, kim2018bayesian}.  
%applications in various  

However, the theoretical properties of SVGD are still largely unexplored. 
%
The only exceptions are \citet{liu2017stein, lu2018scaling},
which studied the partial differential equation that governs the evolution of the limit densities of the particles, with which the convergence to the distribution of interest can be established. 
%
However, the results in \citet{liu2017stein, lu2018scaling} are asymptotic in nature and hold only when the number of particles is very large. 
%
A theoretical understanding of SVGD in the finite sample size region is still missing and 
of great practical importance, 
because the particle sizes used in practice are often relatively small, 
%it has been found that SVGD tends to perform well with a small  practice size 
given that SVGD with a single particle exactly reduces to finding the mode (a.k.a.
maximum a posteriori (MAP)).

\textbf{Our Results}~~ 
We analyze the finite sample properties of SVGD. 
%
In contrast to the dynamical perspective of \citet{liu2017stein}, 
we directly study what properties 
a set of particles would have if it satisfies the fixed point equation of SVGD, 
regardless of how we obtain them algorithmically, 
or whether the fixed point is unique. 
%
Our analysis indicates that the fixed point equation of SVGD is essentially a moment matching condition which ensures that the fixed point particles $\{\vx_i^*\}_{i=1}^n$ \emph{exactly} estimate the expectations of all the functions in a special function set $\F^*$, %of test functions, 
$$\frac{1}{n}\sum_{i=1}^nf(\vx_i^*) = \E_p f, ~~~~~\forall f\in \F^*.$$
This set $\F^*$, which we call the \emph{Stein matching set}, consists of functions obtained by applying Stein operator on the linear span of feature maps of the kernel used by SVGD.  

This framework allows us to understand properties of different kernels 
%Under this framework, we should engineer the kernels 
(and the related feature maps) 
by studying their Stein matching sets $\F^*$, which should ideally either match the test functions that we are actually interested in estimating, or is as large as possible to approximate the overall distribution. 
This process is difficult in general, but we make two  observations in this work: 

\emph{i}) We show that, by using linear kernels (features), SVGD can \emph{exactly} estimate
the mean and variance of Gaussian distributions when the number of particles is larger than the dimension. 
Since Gaussian-like distributions appear widely in practice, and the estimates of mean and variance are often of special importance, linear kernels can provide a significant advantage over the typical Gaussian RBF kernels, especially in estimating the variance. %\todo{wording}
%This highlights the importance of linear kernels because Gaussian-like distributions appear widely in Bayesian inference, and the estimates of mean and variance are of common importance. In fact, empirical results show that SVGD with the typical Gaussian RBF kernel tends to underestimate the variance in high dimensions, a problem can be resolved using linear kernels. 

\emph{ii}) Linear features are not sufficient to approximate the whole distributions.  
We show that, by using random features of strictly positive definite kernels, 
%we develop an $\tildeO(1/\sqrt{n})$ error bound on related kernel Stein discrepancy, which %we show that
the fixed points of SVGD approximate the whole distribution with an $O(1/\sqrt{n})$ rate in kernelized Stein discrepancy. 
%In practice, 

%These two observations motivate us to propose a simple linear+random kernel to combine the advantages of linear and random Fourier features. We perform an extensive empirical study to verify our theoretical results and demonstrate the practical advantages of the linear+random kernel. 
%to get the benefits of both, whose practical advantage is demonstrated using empirical studies. 

%More generally, 
%the ideas developed in this work 
%In additional to 
%Beyond the technical results, 
%our results suggest 
Overall, our framework reveals a novel perspective that reduces the inference problem to either 
a \emph{regression problem} of fitting Stein identities,  
or \emph{inverting the Stein operator} which is framed as solving a differential equation called Stein equation. 
%or a problem of solving a differential equation to invert the Stein operator. 
These ideas are significantly different from 
%It is a significantly different idea from 
the traditional MCMC and VI that are currently popular in machine learning literature, and draw novel  connections to Quasi Monte Carlo and quadrature methods, among other techniques in applied mathematics. 
%
New efficient approximate inference methods may be motivated with our new perspectives.  


==> icml2017/tex/random_perspective.tex <==
\newpage\clearpage


\paragraph{A Perspective from Random Features} 
%It is common that 
Many positive definite kernels admit a random feature representation: 
\begin{align}\label{randk}
k(\vx,\vx') = \E_{w\sim p_w} [\ff(\vx, w) \ff(\vx', w)],
\end{align}
where $\{\ff(\vx,w), ~\forall w\}$ is a feature map indexed by a random parameter $w$ drawn from distribution $p_w$. 
In particular, Borcher's theorem showed that any stationary continuous kernel $k(\vx,\vx') = k(\vx - x')$ admits random Fourier feature $\ff(\vx, w) = \cos(w_1^\top x + w_0 )$ where $w_0\sim \text{Unif}([0,2\pi])$ and the distribution of $w_1$ depends on the kernel \citep{rahimi2007random}. 
%where  $w_1 \sim \normal(0, I_{d\times d})$ 
%and $w_0 \sim Uniform([0,\pi])$?????. 
%But non-stationary kernels also have random feature expansion, such as $\sigma(w^\top x)$. 

With the random feature expansion \eqref{randk}, the kernel Stein discrepancy in \eqref{ksdkernel}  can be rewritten into 
\begin{align}\label{ksdw}
\D^2(q~||~p) =   \E_{w
\sim p_w} \bigg [\left ||\E_{x\sim q} [\steinpx \ff(\vx, w)]\right{||}^2 \bigg ]. 
\end{align}
$\D^2(q~||~p)$ can be viewed as mean square error of Stein identity 
$\E_{x\sim q} [\steinpx \ff(\vx, w)] = 0$ over the random features. 
%Therefore, if $\D^2(q, p) = 0$, it  implies that Stein's identity $\E_{x\sim q} [\steinpx \ff(\vx, w)] = 0$
%simultaneously holds almost surely all the features $\ff(\vx, w)$. %, except a zero probability set (in terms of $p_w$). 
$\D^2(q~||~p) = 0$ shall imply $q = p$ if the random feature set is broad enough. 

Note that the function space $\H$ and the set of random features $\mathcal G = \{\ff(\vx, w)\colon \forall w\}$ 
are different. Stein discrepancy can be viewed as  an \emph{expected} loss function on $\mathcal G$ as shown in \eqref{ksdw}, 
but a \emph{worst-case} loss on $\H$ as shown in \eqref{ksdopt}.  

\paragraph{Stein's Identity as a  Tool for Approximate Inference}
%
A key point of this work is to leverage Stein's identity as a foundation for approximate calculation of integrals. 
%
We consider the problem of finding a set of points (or particles) $\{\vx_i^*\}_{i=1}^n$, 
such that its empirical measure $\hat\mu_n^*(\vx) = \sum_{i=1}^n \delta(\vx-{\vx_i})/n$ approximates $p$ in the sense that $\E_{\hat \mu_n^*} f \approx \E_{p} f$ for a large set of test functions $f$. 

Considering $\T^p\G := \{\steinpx \ff(\vx, w): \forall w\}$ as the set of test function whose expectation is identically zero according to Stein's identity, 
%From Stein's identity perspective, 
the problem amounts to finding a set of points such that Stein's identity holds (approximately):%\begin{box}
\begin{align}\label{findx}
\text{\it Find $\{\vx_i^*\}_{i=1}^n$ s.t. }~~~~ \frac{1}{n}\sum_{i = 1}^n \steinpx \ff(\v\vx_i^*, w) \approx 0, ~~~~ \forall w. 
\end{align}
One possible approach to achieve this is to find $\{\vx_i^*\}$ by explicitly minimizing
the Kernel Stein discrepancy, which is the mean square error according to \eqref{ksdw}, 
$$
\min_{\{\vx_i\}_{i=1}^n}\bigg\{\S^2(\hat\mu_n, ~ p) = \frac{1}{n^2}\sum_{ij=1}^n \kappa_p(\v\vx_i,\v\vx_j) \bigg\}. 
$$
This amounts to an optimization over the particle locations $\{\vx_i\}_{i=1}^n$, which can be solved, for example, using gradient-based methods. 
However, this induces a non-convex optimization problem and does not yield good practical performance as find with empirical experiments.  
A better approach is based on Stein variational gradient descent (SVGD) that we introduce in the sequel, which can be viewed as a fixed point algorithm for achieving \eqref{findx}. 



\section{Choice of $\F^*$}

In this view, the performance of SVGD critically depends on, if not fully determined by, the set $\F^*$. Ideally, we shall design the algorithm (mostly by choosing a proper kernel) such that 
$\F^*$ serves our purpose in either of the two following ways:

1. \emph{Query-specific Inference}. When it is of interest to estimate $\E_pf_0$ of a particular function $f_0$, we should design the algorithm such that $f_0$ is in $\F^*$, or $\F_\epsilon^*$ with small $\epsilon$. 

2. \emph{Distributional Inference}. When it is of interest to have $\hat\mu_{X^*}$ serve an approximation to distribution $p$, e.g., in the sense of weak convergence. We should choose $k(x,x')$ so that $\F^*_\epsilon$ is as large as possible. Ideally, if we can include in $\F^*_\epsilon$ the set of bounded continues functions then $\hat \mu_{X^*}$ weakly converges to $p$. \red{(todo)}

Unfortunately, $\F^*$ depends on both the kernel $k(x,x')$, the Stein operator $\steinpx$ of the target distribution $p$ as well as the fixed points $\{x_i^*\}$ in a complex fashion, which makes it difficult to design algorithm to steer $\F^*$ towards what we want, or perform theoretical analysis. 

1. The dependency on the Stein operator $\steinpx$ seems to be related to the difficult nature of the problem, and can not be sidestepped trivially. This is related what is called \emph{Stein equation} which we believe relate to the heart of inference: 
for a given $f_0$, we can find a $g$ and a constant $c$ such that 
$$f_0 = \steinpx g + c,$$ then we have $\E_{p} f_0 = c$. This transforms the integral problem of calculating $\E_p f_0$ to solving a differential equation. Unfortunately, Stein equation generally requires numerical methods to solve, except for simple Gaussian cases which we show have closed form solution (Section~\ref{sec:gaussian}). 
%Specifically 
%Specifically, 

2. The dependence on the fixed point $\{x_i^*\}$, on the other hand, 
seems to due to the design choice of the SVGD algorithm, and can be sustantially eliminated. In the next section, we show that when $k(x,x')$ is the inner product of a finite number of featues, then $\F$ is the linear span of $\{\steinpx \phi_\ell(x) \colon \ell \in [m]\} \cup \{1\}$.  

%The set $\F^*$  The set $\F_{X^*}$ in Lemma~\ref{lem:exact} depends on the target distribution $p$, the kernel $k(x,x')$ and the fixed point $X^*$. Out of these three factors, the only factor that can be chosen freely is the kernel. However, because of the complexity of the form, it is in general difficult to steer the choice of kernel to make $\F_{X^*}$ matches the function that we want, for example, $x$ and $x^2$. In the following, however, we show that when $p$ is a Gaussian distribution, we can use a polynomial kernel $k(x,x') = x^\top x'$ to make $\F_{X^*}$ include all the first and second order moments. 

%The quality of SVGD approximate critically dependents on $\F_*$, whose choice 

%1. Extending this result, SVGD provides increasingly better approximation when a given $f$ is \emph{close} to $\F_{X^*}$. %This suggests that SVGD is a 

%2. The disadvantage, however, is that the set $\F_{X^*}$ depends on the fixed point $X^*$ itself and can not be specified before hand.  

%3%. This provides a valuable point for \emph{query-specific}
%inference. There is, given a function $f$ of interest, 
%we should design the kernel such that it lies (or approximately lies) in the $\mathcal F$. In the following, we show that for special distributions and test functons, it is possible to design this explicitly.  For general cases, however, we discuss how this can be achieved using random feature and learning theory.  


%In order to 

\paragraph{Stein's Identity as a  Tool for Approximate Inference}
%
A key point of this work is to leverage Stein's identity as a foundation for approximate calculation of integrals. 
%
We consider the problem of finding a set of points (or particles) $\{\vx_i^*\}_{i=1}^n$, 
such that its empirical measure $\hat\mu_n^*(\vx) = \sum_{i=1}^n \delta(\vx-{\vx_i})/n$ approximates $p$ in the sense that $\E_{\hat \mu_n^*} f \approx \E_{p} f$ for a large set of test functions $f$. 

Considering $\T^p\G := \{\steinpx \ff(\vx, w): \forall w\}$ as the set of test function whose expectation is identically zero according to Stein's identity, 
%From Stein's identity perspective, 
the problem amounts to finding a set of points such that Stein's identity holds (approximately):%\begin{box}
\begin{align}\label{findx}
\text{\it Find $\{\vx_i^*\}_{i=1}^n$ s.t. }~~~~ \frac{1}{n}\sum_{i = 1}^n \steinpx \ff(\v\vx_i^*, w) \approx 0, ~~~~ \forall w. 
\end{align}
One possible approach to achieve this is to find $\{\vx_i^*\}$ by explicitly minimizing
the Kernel Stein discrepancy, which is the mean square error according to \eqref{ksdw}, 
$$
\min_{\{\vx_i\}_{i=1}^n}\bigg\{\S^2(\hat\mu_n, ~ p) = \frac{1}{n^2}\sum_{ij=1}^n \kappa_p(\v\vx_i,\v\vx_j) \bigg\}. 
$$
This amounts to an optimization over the particle locations $\{\vx_i\}_{i=1}^n$, which can be solved, for example, using gradient-based methods. 
However, this induces a non-convex optimization problem and does not yield good practical performance as find with empirical experiments.  
A better approach is based on Stein variational gradient descent (SVGD) that we introduce in the sequel, which can be viewed as a fixed point algorithm for achieving \eqref{findx}. 








When using a finite number of features as in Theorem~\ref{thm:phi}, 
the set $\F^*$ is finite dimensional.
How can we extend the result to establish bounds for functions outside of $\F^*$? 
This can be done by using random features drawn from a population, 
%randomly from a p
which allows us to \emph{generalize} the bound to the set of \emph{infinite} mixtures of features with
with $O(1/\sqrt{m})$. 
%$f(x) = \E_w [c_f(w)\steinpx \phi(x,w)]$, 
%which can be approximated by $\F^*$ with accuracy $O(1/\sqrt{m})$, suggesting that $\E_{\mu_{X^*}} f - % \E_pf =O(1/\sqrt{m})$ for these functions. 

Specifically, we draw  $m$ random features $\phi(x, w_\ell)$ with $w_\ell$ drawn i.i.d. from $p_w$. 
%where the number of features 
%yielding a kernel 
This yeilds a kernel $\hat k(x,x') = \sum_{\ell=1}^m \phi(x, w_\ell) \phi(x', w_\ell)$ 
which we then use $\hat k(x,x')$ to run a SVGD with $n$ particles. 
%We assume the number of features $m$ equals or is smaller than 
%$n$, so that the rank of matrix $\Phi=[\phi_\ell(x_i^*)]_{\ell,i}$ in Theorem~\ref{thm:phi} can be $m$.  
Following Theorem~\ref{thm:phi} (assuming the full rank condition holds),   
the fixed point $X^*$ of SVGD should exactly estimates all functions in the linear span $\F^*$ of $\{\steinpx \phi(x,w_\ell), \ell \in [m]\} \cup \{1\}$. 
However, this can be extended to the whole features of features, which is the linear span of
%\{\}
$\{\steinpx \phi(x,w_\ell), \forall w \} \cup \{1\}$. 

We establish two results: 

1. Consider functions of form 
\begin{align}\label{fcf}
%\F_{\infty}^* = \{x\mapsto  \E_{w} [\vv c_f(w)^\top \steinpx\phi(x, w)] \colon ~~~ \sup_w || \vv c_f(w)||_\infty\leq \infty \}. 
f(x) = \E_{w} [\vv c_f(w)^\top \steinpx\phi(x, w)],
\end{align}
for which we may definite a norm $||f||_{\infty,w}:= \inf_{\vv c_f} \sup_w || \vv c_f(w)||_\infty$, 
where the $\inf$ is taking over all $\vv c_f$ that satisfies \eqref{fcf}. 
Define $\F_\infty^*$ to be the set of functions $f$ with $||f ||_{\infty, w}<\infty$, 
then we can show that the fixed points of SVGD approximats $\E_p f$ for functions in $\F_{\infty}$ 
with $O(1/\sqrt{m})$ accuracy. 
%
%

%For convenience, we denote by $\phi_p(x,w) = \steinpx\phi(x,w)$. 
   \begin{ass}\label{ass:ass}
  1)  Assume $\{\phi(x,w_\ell)\}_{\ell=1}^m$ is a set of random features with $w_\ell$ i.i.d. drawn from $p_w$ on domain $\W$, and $X^*= \{x_i^*\}_{i=1}^n$ is an \emph{approximate} fixed point of SVGD with random feature $\phi(x,w_\ell)$ in the sense that 
$$
||\frac{1}{n}\sum_{i=1}^n \steinpx \phi(x_i^*, w_\ell)||_1 \leq \frac{\epsilon}{\sqrt{m}}.  
$$
2) We have $ \sup_{x \in \mathcal X}  \sup_{w\in \W} |\steinpx\phi(x, w)|  = M_{\psi_p} < \infty$. This may imply that $\mathcal X$ has to be compact since $\nabla_x \log p(x)$ is typically unbounded on non-compact $\X$ (e.g., when $p$ is standard Gaussian,$\nabla_x \log p(x) = x$). 

4. Define function set 
$$\stein\Phi = \{ w \mapsto   \stein_{x^\ell}\phi(x, w)  \colon  \forall x \in \X, ~~ \ell \in [d]  \},$$
where $\stein_{x^\ell}$ denotes the stein operator w.r.t. the $\ell$-th coordinate $x^\ell$ of $x$ 
We assume the Rademacher complexity of $\stein\Phi$ satisfies $R_m(\stein \Phi) \leq R_p/ \sqrt{m}.$ 
\end{ass}

\begin{thm}\label{thm:fxbound}
Under Assumption~\ref{ass:ass}, 
for any given function $f$ in $\F_\infty^*$ defined in \eqref{fcf}, 
we have with at least probability $1-\delta$ (in terms of the randomness of $\{w_\ell\}$), 
$$
\left |\frac{1}{n}\sum_{i=1}^n f(x_i) - \E_p f \right |
\leq   \frac{C(1  + \epsilon +  \sqrt{2\log (1/\delta)})}{\sqrt{m}},
%\leq  \frac{M_1 +  M_v M_{\psi_p}\sqrt{2\log (1/\delta)}}{\sqrt{m}},
$$
where $C$ is a constant %independent of $n$ and $m$, 
that depends on $R_p$, $M_v$ and $M_{\psi_p}$ defined in Assumption ~\ref{ass:ass} below. 
%Specifically, $C = \max(4(R_p + M_v)( M_{\psi_p} + M_v),~ M_v)$ defined in Assumption ~\ref{ass:ass} below. 
%depends on the $$
%M = 4(R_p + M_v)( M_{\psi_p} + M_v) + \epsilon M_v$. 
\end{thm}
\remark{Note that this is not a uniform bound, that is, it does not bound $\sup_{f\in F}|\frac{1}{n}\sum_{i=1}^n f(x_i) - \E_p f | $. We need to bound KSD  directly in order to get the uniform bound.}

\remark{The convergence rate is expressed in terms of the feature size $m$, not the particle size $n$. However, in order to satisfy the moment equations for $m$ features, there must be at least $n$ particles. We set $n = m$ in most of the cases.}





\section{Convergence rate of Stein Discrepancy}

\begin{thm}\label{thm:unibound}
Under Assumption~\ref{ass:ass}, for any $\delta > 0$, we have with  at least  probability $1-\delta$,  
$$
%\sup_{f\in \H_p^+}\{ \E_{X^*} f - \E_pf\} = 
%\S(\hat\mu_{X^*}, p)^2 \leq 
\S^2(\hat\mu_{X^*}, p) \leq  \frac{C}{m}\bigg [ \epsilon^2 + \log^{3}m  + {\log(1/\delta) \bigg]
%= O\bigg (\frac{\log^{1.5} m}{\sqrt{m}} \bigg).
$$
%More specifically, 
%$$
%\S^2(X, p) \leq  \frac{1}{m}\bigg [ \epsilon^2 +
 %K\bigg (    \epsilon  \sqrt{2} \log^{1.5} m  {R_p} 
%+ \epsilon \sqrt{{M_{\psi_p}^2\log(1/\delta)}}  + 2\log^{3}m {R_p^2} + {M_{\psi_p}^2\log(1/\delta)} \bigg) \bigg]. 
%$$
where $C$ is a constant depends on $R_p$ and $M_{\psi_p}$. 
%where $K < 10^5$ is a numerical constant defined in Theorem~XX of \citet{srebro2010smoothness}. 
\end{thm}
\remark{It is unclear if the $\log^{1.5} m$ term can be eliminated, but it would be supervised that it is the cost to pay in order to get a uniform bound compared to the result in Theorem~\ref{Ef}.}
\remark{Similar to the proof of Theorem~\ref{thm:fxbound}}, 
the proof of \ref{thm:unibound} relies on generalization bounds from statistical learning theorem. To build the connection, 
define $g_X(w) = \hat \E_X[\psi(X, w)],$ we can view $g$ as a hypothesis class with $w$ as the data, and $X$ as the parameter. 
Assume each $w$ is associated with a label that is identically equal to zero, then the expected quadratic loss function is 
$$
\S^2(X, p) = \E_{w} [(g_X(w))^2]. 
$$
In random feature SVGD, however, we draw random $\{w_i\}_{i=1}^m$ and select $X$ such that $g_X(w_i) \approx 0$. This defines an empirical loss function: 
 $$
\hat \S^2(X, p) = \frac{1}{m}\sum_{i=1}^m  [(g_X(w_i))^2].  
$$
We are interested in bounding the expected loss $\S^2(X, p)$, because it is the maximum mean discrepancy for all functions in $\H_p^+$: 
$$
\S(X, p) = \sup_{f\in \H_p^+} \big\{\frac{1}{n}\sum_{i=1}^n f(x_i) - \E_pf \big\}. 
$$
As in typical learning theory, the expected loss can be bounded by 
%$\S^2(X, p)$
the empirical loss $\hat \S^2(X, p)$ (which we assume is $O(1/\sqrt{m})$) and the generalization bound 
that controls the difference between the empirical and expected loss uniformly over all hypothesis $g_X$.  
If we apply standard generalization bound, 
we would have $\S^2(X, p) \leq \hat \S^2(X, p) + O(1/\sqrt{m}) = O(1/\sqrt{m})$, 
which implies $\sup_{f\in \H_p^+} \big\{\frac{1}{n}\sum_{i=1}^n f(x_i) - \E_pf \big\} = \S(X^*, p) = O(1/m^{1/4})$.
This, however, is does not reach the typical $1/\sqrt{n}$ rate. 

Fortunately, the  excess risk can be shown to be $O(1/m)$ when the noise is low, which is exactly our case (we know that the true labels are exactly zero). 
In particular, we use the bound in  \citet{srebro2010smoothness}. These bounds are often proved using local Radermacher complexity \citep{bartlett2005local}. 


Our results require to bound the Rademacher complexity $R_m(\Psi_p)$ of the Steinalized features $\Psi_p = \{ w\mapsto \psi_p(x, w) \colon x \in \X\}$. Recall that 
$$
\psi_p(x, w) = \steinpx \psi(x, w) = \nabla_x \log p(x) \psi(x, w) + \nabla_x \psi(x, w). 
$$
Therefore, it is enough to bound  the Rademacher complexity of $\Psi$ and $\nabla_{x_\ell} \Psi$, $\forall i=1,\ldots, d$. 
\begin{lem}
Define $\Psi = \{w \mapsto \phi(x, w) 
\colon \forall x \in \mathcal X\}$ and $\nabla_{x_\ell} \Psi = \{w \mapsto \nabla_{x_\ell} \phi(x, w)  \colon \forall x \in \mathcal X\}$, for each coordinate $\ell = 1,\ldots, d$. Then
$$
R_m(\steinpx^\ell \Psi ) \leq ||  \nabla_{x_\ell} \log p ||_\infty R_m (\Psi )  + R_m(\nabla_{x_\ell} (\Psi)), 
$$
where $|| \nabla_{x_\ell} \log p||_\infty  = \sup_{x\in \X} |\nabla_{x_\ell} \log p(x) |$. 
\end{lem}
Therefore, it is enough to bound $R_m(\Psi)$ and $R_m(\nabla_{x_\ell} \Psi)$, $\forall i=1,\ldots, d$. 
We consider a number of cases. 
\begin{itemize}
\item $\psi(x,w)  = \sigma(w^\top x)$ where $\sigma$ is a $L_\sigma$-Lipschitz function, then 
$$
R_m(\Psi) \leq \frac{1}{\sqrt{m}}  \big( 2 L_\sigma || \mathcal X||_{2,\infty} \sqrt{\E_w[||w ||_2^2]} + \sigma(0) \big). 
$$ 
where $|| \mathcal X||_{2,\infty}  = \sup_{x\in \mathcal X} || x||_2$. 

In addition, assume the derivative $\sigma'$ is also Lipschitz, we have $\nabla_{x_\ell} \psi(x,w) = w_\ell \sigma'(w^\top x)$. Then from Lemma~\ref{lem:fg} 5), 
$$
R_m(\nabla_{x_\ell} \Psi) \leq \frac{1}{m}(M_{\sigma'}  +  \max_i w_{i,\ell} )( 2 L_{\sigma'} ||\mathcal X ||_{2,\infty} \E_w || w_2||^2 + \sigma'(0) + \max_{i} w_{i,\ell} )
$$
\red{Better bounds? for product of two functions, or for derivative? Understand the proof of Lipschitz Rademacher?} 

Using L1 norm instead. Define $|| \X ||_{1,\infty} = \sup_{x\in \X} \{ ||x ||_1 \}$. 
Consider $G = \{w \mapsto x^T w \colon ||x ||_1 \leq M_x\}$, then 
Then
$$
R_m  (G) \leq \frac{M_x \max_i ||w_i||_\infty \sqrt{2 \log (2d)}}{\sqrt{m}}. 
$$

$$
R_m(\nabla_{x_\ell} \Psi) \leq \frac{1}{m}\E_w (M_{\sigma'}  +  \max_i || w||_\infty )( 2 L_{\sigma'} ||\mathcal X ||_{1,\infty} \max_{i}||w||_\infty+ \sigma'(0) + \max_{i} ||w||_\infty)
$$

\end{itemize}


\paragraph{Main Results}
We develop a quick technical review of the main idea of this paper. 
Under Stein's method \citep{stein1972}, a distribution $p$ is uniquely characterized by its related Stein operator $\steinpx\ff(x) = \nabla_\vx \log p(\vx) \ff(x) + \nabla_\vx \ff(x)$, for which Stein's identity holds:  $\E_p[\steinpx \ff(x)] = 0$ for any function $\ff$. 
%which is a linear functional operator apply on function $\ff$. 
SVGD finds a set of particles $\{\vx_i\}_{i=1}^n$ for approximating $p$ 
by iterative updates of form: 
\begin{align}\label{up0}
\vx_i \gets \vx_i + \frac{1}{n}\sum_{j=1}^n\steinpx k(\vx_j, \vx_i). 
\end{align}
where $k(\vx, \vx')$ is any positive definite kernel, which is assumed to be spanned by a finite number of features:  $k(\vx,\vx') = \frac{1}{n}\sum_{\ell=1}^n \phi_\ell(\vx)\phi_\ell(\vx')$. 
For any fixed point $\{\vx_i^*\}$ of SVGD, 
we show that once matrix $\Phi = [\phi_\ell(x_i^*)]_{\ell, i}$ is full rank (which can be verified numerically), 
 we have 
$$
\frac{1}{n}\sum_{i=1}^n f(\vx_i^*) = \E_{p} f, ~~~ \forall f\in \F^*,
$$
where $\F^*$ is the set of functions of form $f(x) = \steinpx \ff(\vx) + b$ where $b\in \RR$   and $\ff$ is any function in the linear span of $\{\phi_\ell\}$, that is,  $\ff(\vx) = \sum_{\ell=1}^n \vv a  \phi_\ell(\vx)$, $\forall \vv a_\ell \in \RR^d$. 
Having this set up,
we want to choose the features and the kernel so that $\F^*$ matches the functions of particular interest, or make $\F^*$ as large as possible to obtain distributional approximation. 
Although it is generally difficult to infer what feature $\phi_\ell$ is needed to do exactly estimate a given function $f$ (this process is called solving Stein equation), in the special case of Gaussian, we prove a simple result that using lienar features allows us to exactly recover both the mean and variance of Gaussian. This suggests that it is good to use linear kernels for Gaussian-like distributions (which appears widely in typical Bayesian inference tasks). 

Also, we show that by using random features $\phi_\ell(\vx) = \phi(\vx,\vw_\ell)$ where $\vw_\ell$ is a random parameter drawn from a distribution $p_w$, we can establish a bound of $\sup_{f\in \H_p^+} \{\E_{\hat\mu_{X^*}} f - \E_p f\} = \tilde O(1/\sqrt{n})$, where $\H_p^+$ is the set of functions of form $f(x) = \steinpx^\top \ff(x) + b$, $\forall b \in \RR$ and $\ff$ is any function in the RKHS $\H^d$ with positive definite kernel $k(\vx,\vx') = \E_{w\sim p_w}[\phi(\vx, \vw) \phi(\vx', \vw)]$. 

%We first show that 
%to obtain a
%When $\ff$ is Gaussian. We can show that 
%Therefore, 
%We show that 
%$k(x,x') = $
%We consider kernels 
%Assume $k(x,x')$


==> icml2017/tex/randomfeaturesvgd.tex <==

\subsection{Random feature SVGD}\label{sec:random}
The linear features are not sufficient for providing the consistent estimation of the whole distribution, even for Gaussian distributions.  
Non-degenerate kernels are required to obtain bounds on the whole distributions, but they complicate the analysis because their Stein matching set depends on the solution $X^*$ as shown in Lemma~\ref{lem:fg}. 
%In order to obtain asymptotic consistency theoretically, we need to a systematic way to include more  linearly independent features as we use more particles. 
Random features can be used to sidestep this difficulty \citep{rahimi2007random}, enabling us to analyze a random feature variant of SVGD with probabilistic bounds. 
%This can be achieved using the idea of random features \citep{rahimi2007random}. 
%Random features have alo been widely used to speed up computation in kernel method, 
%including 
%our motivation, how
%of positive definite kernels, %a technique that has been widely used in kernel learning  


To set up, assume $k(\vx,\vx')$ is 
a universal kernel whose Stein discrepancy $\D_k(q~||~p)$ yields a discriminative measure of differences between distributions. 
%
Assume $k(\vx, \vx')$ yields the random feature representation in \eqref{kphi}, and we can approximate it %with a 
%
%We analyze the SVGD which 
%, instead of using 
%Instead of running SVGD directly with 
%kernel $k(\vx,\vx')$, 
%approximate it with 
%a degenerated kernel with 
by drawing $m$ random features,  %$(m\leq n)$,   
$$
\hat k(\vx,\vx') = \frac{1}{m}\sum_{\ell=1}^m {\phi}(\vx, \vw_\ell) \phi(\vx', \vw_\ell),
$$
where $\vw_{\ell}$ are i.i.d. drawn from $p_\vw$. 
% SVGD with kernel $\hat k(\vx, \vx')$. 
We assume $m\leq n$, then running SVGD with kernel $\hat k(\vx, \vx')$ (with the random features fixed during the iterations) yields a matching set that decouples with the fixed point $X^*$. 
In this way, our result below establish that 
%for any fixed point $X^*$, we have
$\D_k(\hat\mu_{X^*}~||~p) = \tilde O(1/\sqrt{n})$ with high probability. According to \eqref{shp}, this provides a uniform bound of $\E_{\hat\mu_{X^*}}f-\E_pf$ for all functions in the unit ball of $\H_p^+$. 

Here, random features are introduced mainly for facilitating theoretical analysis, 
but we also find random feature SVGD works comparably, and sometimes even better than SVGD with the original non-degenerate kernel (see Appendix). This is because with a finite number $n$ of particles, at most $n$ function basis of $k(x,x')$ can be effectively used, even if $k(x,x')$  itself has an infinite rank. 
From the perspective of moment matching, 
there is no benefit to use universal kernels when the particle size $n$ is finite. 
%The intuition is that we 
%although 
%This means that \{$w_\ell\}$ are drawn in the beginning an1d fix it during the SVGD iterations. 
%In this way, fixed point of SVGD  achieves that $\hat D_{k}(\hat \mu_{X^*} ~||~ p) = 0$ if the rank condition holds. However, unlike $\D_{k_\infty}$, $\D_{k}$ is not a  discriminative and does not bound the difference of  $\mu_{X^*}$ and $p$ as distributions.  However, thanks to the generalizability of the random features, we show in Theorem~\ref{thm:unibound} $$\D_{k_\infty}(\mu_{X^*}~||~p) =  \sup_{f\in \H_p^+} |\E_{\mu_X^*} f - \E_p f | = \tilde O(1/\sqrt{m}).$$ 

%Before introducing the technical details of our result,  we 
In the sequel, we first explain the intuitive idea behind our result, highlighting a perspective that views inference as fitting a zero-valued curve with Stein's identity, and then introduce technical details. 

%To develop the intuitive idea, we observe that with the random feature expansion \eqref{randk}, the kernel Stein discrepancy in \eqref{ksdkernel}  can be rewritten into 
%\begin{align}\label{ksdw}
%\D^2(q~||~p) =   \E_{w
%\sim p_w} \bigg [\left ||\E_{x\sim q} [\steinpx \ff(\vx, w)]\right{||}^2 \bigg ]. 
%\end{align}
%$\D^2(q~||~p)$ can be viewed as mean square error of Stein identity 
%$\E_{x\sim q} [\steinpx \ff(\vx, w)] = 0$ over the random features. 
%Therefore, if $\D^2(q, p) = 0$, it  implies that Stein's identity $\E_{x\sim q} [\steinpx \ff(\vx, w)] = 0$
%simultaneously holds almost surely all the features $\ff(\vx, w)$. %, except a zero probability set (in terms of $p_w$). 
%$\D^2(q~||~p) = 0$ shall imply $q = p$ if the random feature set is broad enough. 
%Note that the function space $\H$ and the set of random features $\mathcal G = \{\ff(\vx, w)\colon \forall w\}$ 
%are different. Stein discrepancy can be viewed as  an \emph{expected} loss function on $\mathcal G$ as shown in \eqref{ksdw}, 
%but a \emph{worst-case} loss on $\H$ as shown in \eqref{ksdopt}.  
\newcommand{\Xs}{{X^*}}
\newcommand{\vxs}{x^*}
\textbf{Distributional Inference as Fitting Stein's Identity} 
Recall that our goal can be viewed as finding  particles $\Xs=\{\vx_i^*\}$  such that their empirical 
$ \hat\mu_{\Xs}$ 
approximates the target distribution $p$. 
We re-frame this into finding $\hat\mu_\Xs$ such that Stein's identity holds (approximately): 
\begin{align*}
    \text{Find $\hat\mu_{\Xs}$} && s.t. &&  \E_{\hat\mu_{\Xs}}[\steinpx \phi(\vx,\vw)]\approx 0, ~~~ \forall \vw. 
\end{align*}
%More specifically, define $$
%T
%In order to make $\mu_{X^*}$ match, we should set $X^*$ such that $\steinpx \phi(\vx, w) = 0$ for all $w$ (the Stein identity). 
%This can be viewed as a special supervised learning problem:
We may view this as a special curve fitting problem: considering $\vv g_{X}(\vw) = \E_{\hat\mu_X} [\steinpx \phi(\vx,\vw)]$, we want to find ``parameter'' $X$ such that $\vv g_X(\vw) \approx 0$ for all inputs $\vw$. 
The kernelized Stein discrepancy (KSD), as shown in \eqref{ksdw}, 
can be viewed as the expected rooted mean square loss of this fitting problem:
\begin{align}
\label{gxD}
\D_k^2(\hat\mu_X~||~p) = 
%\left (
%\sqrt{ 
\E_{\vw\sim p_\vw}\left [||\vv g_X(\vw)||^2_2\right ] 
%}
%\right)^{1/2}. 
\end{align}
%Our random feature approach can be viewed as an \emph{empirical risk minimization} approach \citep{vapnik2013nature}, which minimizes 
When replacing $k(\vx,\vx')$ with its random feature approximation $\hat k(\vx, \vx')$, the corresponding KSD can be viewed as an empirical loss on random sample $\{\vw_\ell\}$ from $p_\vw$: 
$$
\D_{\hat k}^2(\hat\mu_X ~||~p) = 
%\left (
%\sqrt
{\frac{1}{m}\sum_{\ell=1}^m 
\left [||\vv g_X(\vw_\ell)||^2_2\right ] }.% \right)^{1/2}.  
$$
By running SVGD with $\hat k(\vx,\vx')$, 
we acheive $\vv g_{X^*}(\vw_\ell)=0$ for all $\ell$ at the fixed point, implying  
a zero empirical loss $\D_{\hat k}(\hat\mu_{X^*}~||~p) =0$ assuming the rank condition holds. 
%at the fixed point $X^*$ of SVGD with the empirical kernel $\hat k(\vx,\vx')$, 

The key question, however, is to bound the expected loss $\D_k(\hat \mu_{\Xs}~||~p)$,
which can be achieved using generalization bounds in statistical learning theory. 
In fact, standard results in learning theory suggests that the difference between the empirical loss and expected loss is $O(m^{-1/2})$,  yielding  $\D_k^2(\hat\mu_{\Xs}~||~p)  = O(m^{-1/2})$. 
However, following \eqref{shp}, 
this implies $\E_{\hat\mu_{\Xs}}f - \E_pf=O(m^{-1/4})$ for $f\in\H^+_p$, which does not acheive the standard $O(m^{-1/2})$. 
%bound, which is not tight.  
%
 Fortunately, note that our setting is noise-free, and we achieve zero empirical loss; 
 thus, we can get a better rate of $\D_k^2(\hat\mu_X~||~p)  = \tilde O(m^{-1})$ 
 using the techniques in \citet{srebro2010smoothness}. 
 %which yields, in our setting, 

%It remains to bound the difference between the empirical loss and expected loss,  which can be achieved using uniform concentration bounds in statistical learning theory. Assume the set the Rademacher complexity $R_n(\mathcal G)$ of the hypothesis set $\{\vv g_X \colon \forall X\}$ is $O(1/\sqrt{n})$, which is a natural assumption in learning theory. then the standard generalization bound gives
%A standard generalization bound would allow us to establish  $\D^2(q~||~p) = \D^2(q~||~p) + O(1/\sqrt{m})$.However, because this setting is a low noise setting in that we can get zero empirical loss $\D^2(q~||~p)=0$, and hence we get better bounds:$\D^(q~||~p) = \D^2(q~||~p)  + \tilde O(1/{m})$. 
%the loss function of \emph{learning} problem. 

%For convenience, we denote by $\phi_p(x,w) = \steinpx\phi(x,w)$. 
\textbf{Bound for Random Features} 
We now present our concentration bounds of random feature SVGD. 
   \begin{ass}\label{ass:ass}
  1)  Assume $\{\phi(\vx,\vw_\ell)\}_{\ell=1}^m$ is a set of random features with $\vw_\ell$ i.i.d. drawn from $p_\vw$ on domain $\W$, and $X^*= \{\vx_i^*\}_{i=1}^n$ is an \emph{approximate} fixed point of SVGD with random feature $\phi(\vx,\vw_\ell)$ in the sense that 
$$
|\E_{\vx \sim \hat \mu_{X^*}}\steinp_{x^j} \phi(\vx, \vw_\ell)| \leq \frac{\epsilon_j}{\sqrt{m}}.  
$$
where $\stein_{x^j}$ is the Stein operator w.r.t. the $j$-th coordinate $x^j$ of $\vx$. Assume  $\epsilon^2:=\sum_{j=1}^d\epsilon_j^2 <\infty$. 

2) Let $ \sup_{\vx \in \mathcal X,\vw\in \W} |\steinp_{x^j}\phi(\vx, \vw)|  = M_j$, and $M^2:=\sum_{j=1}^dM_j^2<\infty$. This may imply that $\mathcal X$ has to be compact since $\nabla_{\vx} \log p(\vx)$ is typically unbounded on non-compact $\X$ (e.g., when $p$ is standard Gaussian,$\nabla_{\vx} \log p(\vx) = \vx$). 

3) Define function set 
$$\steinp_j\Phi = \{ \vw \mapsto   \stein_{x^j}\phi(\vx, \vw)  \colon  \forall \vx \in \X \}.$$ 
%where $\stein_{x^\ell}$ denotes the stein operator w.r.t. the $\ell$-th coordinate $x^\ell$ of $x$ 
We assume the Rademacher complexity of $\steinp_{j}\Phi$ satisfies $\Rm(\stein_j \Phi) \leq R_j/ \sqrt{m},$ and $R^2 := \sum_{j=1}^d R_j^2<\infty$.   
\end{ass}

\begin{thm}\label{thm:unibound}
Under Assumption~\ref{ass:ass}, for any $\delta > 0$, we have with  at least  probability $1-\delta$ (in terms of the randomness of feature parameters $\{\vw_\ell\}_{\ell=1}^m$),  
\begin{align}
\label{bdslogm}
\!\!
\!\!\!\! \S_k(\hat\mu_{X^*}~||~p) \leq  \frac{C}{\sqrt{m}}\bigg [ \epsilon^2 + \log^{3}m  + \log(1/\delta) \bigg]^{1/2}, 
\end{align}
where $C$ is a constant that depends on $R$ and $M$.   
\end{thm}
\paragraph{Remark}
Recalling \eqref{shp}, Eq~\eqref{bdslogm} provides a uniform bound 
$$
%\sup_{f\in\H_p^+} \big \{ \E_{\mu_{X^*}} f - \E_p f~~~~~s.t.~~~~||f ||_{\H_p^{+}} \leq 1 \big \} = O(m^{-1/2}{\log^{1.5} m}).
\sup_{||f ||_{\H_p^{+}} \leq 1} \big \{ \E_{\mu_{X^*}} f - \E_p f\big \} = O(m^{-1/2}{\log^{1.5} m}).
$$
This is a uniform bound that controls the worse error uniformly among all $f\in \H_p^+$. 
It is unclear if the logarithm factor $\log^{1.5}m$ is essential. 
In the following, we present a result that has an $O(1/\sqrt{m})$ rate, 
without the logarithm factor, but only holds for  individual functions. 
%Here we an alternative result that have no logarithm factor. 
\begin{thm}\label{thm:fxbound}
Let $\F_\infty$ be the set of linear span of the Steinalized features: 
\begin{align}\label{finfty}
f(\vx) = \E_{\vw\sim p_\vw} [\vv v(\vw)^\top \steinpx \phi(\vx, \vw)], 
\end{align}
where $\vv v(\vw)=[v_1(\vw),\ldots, v_d(\vw)]\in \R^d$ is the combination weights that satisfy $\sup_{\vw} ||\vv v(\vw)||_\infty <\infty$. We may define a norm on $\F_\infty$ by $||f||_{\F_\infty}^2 := \inf_{\vv v} \sum_{j=1}^d\sup_{\vw}  |v_j(\vw)|^2$, where $\inf_{\vv v}$ is taken on all $\vv v(w)$ that satisfies \eqref{finfty}. 

Assume Assumption~\ref{ass:ass} holds, then for any given function $f\in \F_\infty$ with $||f||_{\F_\infty}\leq 1$, we have with at least probability $1-\delta$, 
$$
\left |   \E_{\hat\mu_{X^*}} f - \E_p f  \right   | \leq \frac{C}{\sqrt{m}} (1+ \epsilon + \sqrt{2\log(1/\delta)}), 
$$
where $C$ is a constant that depends on $R$ and $M$. 
 \end{thm}
 The $\F_\infty$ defined above is closely related to the RKHS $\H_p$. 
In fact, one can show that $\F_\infty$ is a dense subset of $\H_p$ \citep{rahimi2008uniform} and is hence quite rich if $k(\vx,\vx')$ is set to be universal. 
 %\citet{} can show that the $\F_\infty$ is a dense subset of 
 %The $\F_\infty$ above 
%\red{todo1}With a different approach, we can establish an $O(1/\sqrt{m})$that holds for individual functions $f$.  
%\red{todo2}%\paragraph{Remark} 
%Discussing Rademacher complexity. The key requirement is that the domain of $x$ and the feature parameter $w$ should be bounded. This seems to be not required for practical purposes. Therefore, a key open direction is to establish requires that does not require compactness on the domain of $x$ and $w$. 




